Enabling Low-power Duplex Visible Light Communication

The new generation of LED-based illuminating infrastructures has enabled a "dual-paradigm" where LEDs are used for both illumination and communication purposes. The ubiquity of lighting makes visible light communication (VLC) well suited for communication with mobile devices and sensor nodes in indoor environment. Existing research on VLC has primarily been focused on advancing the performance of one-way communication. In this paper, we present Retro-VLC, a low-power duplex VLC system that enables a mobile device to perform bi-directional communication with the illuminating LEDs over the same light carrier. The design features a retro-reflector fabric that backscatters light, an LCD shutter that modulates information bits on the backscattered light carrier, and several low-power optimization techniques. We have prototyped the Reader system and made a few battery-free tag devices. Experimental results show that the tag can achieve a 10kbps downlink speed and 0.5kbps uplink speed over a distance of 2.4m. We also outline several potential applications of the proposed Retro-VLC system.

==> ViTag.tex <==
\section{\retro\ Design}

% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/corr-bd.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf System Diagram} (a) \vitag\ and (b) Modified LED.}
% \label{fig:sysdiagram}
% \vskip -0.05in
% \end{figure}

\begin{figure*}[!t]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{cc}
\epsfig{file=../figures/corr-bd.eps, width=\columnwidth} & \epsfig{file=../figures/corr-bd.eps, width=\columnwidth}\\
{(a) \vitag\ Block Diagram} & {(b) LED BLock Diagram}\\
\end{tabular}
}
\vskip -0.1in
\caption{\footnotesize{\bf System Diagram.} Blah Blah.}
\label{fig:sysdiagram}
\vspace{-1em}
\end{figure*}

\retro\ is a new form of communication in which battery-free \vitag\/s can communicate with LEDs without any additional infrastructure. Harvesting LED light energy, a \vitag\ reflects visible light signals to communicate. Because of the ubiquitous deployment of illuminating LEDs, building such a system will enable ubiquitous communications at an unprecedented scale. It will also enhance the security of current RFID systems as it limits the uplink signal exposure to line-of-sight, and the use of retro-reflectors will further focus the signal to an even thiner area, leaving less chance for the hidden attackers and sniffers to temper the system.

Designing such a system, however, faces several challenges, which we will break down in the following subsections, and we describe how our design address these challenges.


%Designing such tags, however, is challenging for four reasons: First, the visible light that carries data is interleaving with intensive interference, such as radios operating at the same frequency, and the light emitted from the LEDs that also carries data and its reflections from surrounding walls, thus making an interference-intensive receiving condition for both \vitag\ and \reader. Second, the signal is exposed to noise, such as the existing environmental lights that is subject to constant changing, human-body-movement-caused noise, and the noise caused by the hardware system itself. Third, to emit modulated light from \vitag\ and make it detectable by \reader\ on a battery-free tag is challenging in that modulating signals on visible light bands is power-consuming with respect to the goal of being battery-free. Finally, to integrate the system to off-the-shelf LED lights while keeping the brightness of the lights constant is challenging. In the rest of this section and the next section, we describe how our design addresses the above challenges.




\subsection{Overview}
Fig.~\ref{fig:sysdiagram} (a) shows a block diagram of our \vitag\ design. It consists of a transmitter, a receiver, an MCU and a harvester. The transmitter and receiver communicate by modulated backscattering of visible light signals, and the harvester absorbs energy from visible lights to power the device. Further, they operate independently of each other. The receiver immediately awakes the MCU by rising the tag voltage to a certain value and enabling the analog circuit to start receiving as it detects a data packet coming in. The MCU then shuts down the analog circuit and powers up the transmitting circuit. The receiving circuit and the transmitting circuit work alternately to save energy. Alongside the communication modules is the energy harvester, which consists of a number of solar cells that transfer visible light energy into electric energy. The harvester sets the upper bound of the power \vitag\ can take on, thus posing a strict constraint to the design of each component on the tag.

Fig.~\ref{fig:sysdiagram} (b) shows a block diagram of our \reader\ design. The major part of it is an LED bulb that emits fast-fluctuating light human eyes cannot detect flickering in. \reader\ builds on off-the-shelf LEDs and makes minor modifications on them. It consists of a transmitter, a receiver and an MCU. The transmitter encodes and modulates the data, feeding the data to the LED for transmission, while keeping the LED not flickering and with dimming support. The transmitter also takes the goal of making \vitag\ battery-free in mind, emitting lights with data such that \vitag\ can demodulate and decode the data at a low energy cost. The receiver deals with the light backscattered from \vitag, and also cancels noise and interference as much as possible. The MCU processes the data transmitted from \vitag.

Next, we describe our design of the transmitter and receiver on the \vitag\ and LED in more detail.





\subsection{\reader\ Transmitter}

As shown in Fig.~\ref{fig:sysdiagram} (b), the transmitter on \reader\ is composed of a crystal oscillator that runs at 1MHz, and an MCU followed by two amplifiers. The data generated by the MCU controls a switch on waves generated by the crystal oscillator so that the data is modulated. The modulated signal will then be amplified and fed to a LED. To make sure the brightness of the LED does not pose a difference between the transmitting and not transmitting state, we add a DC component of a particular value to signal when at the transmitting state such that the the average strength of the light at the transmitting state is the same as solely lighting. The magnitude of the DC component is such that it is adjustable to provide dimming support as what existing LEDs are capable of. In addition to the dimming support, flickers are avoided in \reader\ transmitter. We use 10kHz as the data rate, which far exceeds the frequency (200 Hz) below which human eyes will feel of fluctuations, which could disturbing and unacceptable. 

We note the following about our design: Firstly, we use a white-colored LED, which emits electromagnetic waves of wavelengths between 380 and 780 nm. The highest flickering frequency of the LED  with full on/off transitioning is 1MHz, and we are exploiting the flickering rate to its fullest, in order to leave room for downlink data rate as high as possible. 

Secondly, different components in the transmitter on the reader side require different voltage supply. We are using two DC/DCs to boost the voltage for the switch and the amplifiers. Specifically, the voltage used for supply the crystal oscillator, the amplifiers for the MCU-output signals and the switch is 5V, and the voltage for the amplifiers for the RF signals is 12V. 

Finally, the 1MHz frequency, as mentioned earlier, is used because of the full flickering capability we would like to draw from the LED. However, around this frequency with a bandwidth on the order of 100kHz, there are  commercial radios using AM modulation. For example, there are radios from 540 through 1610 kHz with 10 kHz spacing in America. Another form is situated at a similar spectrum spanning from 531 to 1611 kHz with 9 kHz spacing. These are sources of interference to what we transmit with the LED, and we are going to address this issue with the receiver design on the reader, which also deals with other sources of interference and noise.





\subsection{\vitag\ Receiver}
Looking along the flow of the signal, we then describe the design of our \vitag\ receiver. Designing a visible light receiver entails a light sensor that captures the fluctuation of the visible light with a satisfying bandwidth. Then the captured signals go through filters, detectors/demodulators, and another feedback amplifier before sending to a comparator be digitized. On top of these, the design should be energy-efficient, such that the harvested energy is enough to supply the operation of the tag. We avoid using power-demanding ADCs while achieving \hl{data rate} at \hl{x} accuracy at the distance of \hl{sss} using only analog elements and a low-power MCU. The block diagram of the receiver is presented in Fig.~\ref{fig:sysdiagram} (a).

\subsubsection{Extracting Information from the Visible Light}
\reader\ transmitted signals will first be sensed by a light sensor BPW34. Since the light sensor has an equivalent capacitance, along with an inductor parallel to it, it performs preliminary front-end filtering. Since natural lights do not have a component at 1MHz, this filter does a good job singling out the useful signal and filtering out lights from other sources. Next, two amplifiers will successively increase the RF signal strength while avoiding auto-excitation using feedback mechanisms. After the preliminary filtering and amplification, the signal is ready for demodulation. These processing blocks consume power up to \hl{aaa}, of which the light sensor consumes \hl{ddd}, and they are shut down once the tag turns into the transmitting mode in order to save energy.

Next, we describe the mechanism of our simple yet powerful signal detector under a strict energy constraint. The circuit is a variant of an envelope detector. Unlike a conventional envelope detector, the detector is targeted specifically for energy-constraint conditions, while providing a higher gain and a bigger bandwidth. So it is especially suitable for \vitag, where the downlink data rate is high but with being battery-free as its goal. At a high level, it contains a constant current source, a diode, and a frequency selection amplifier. The constant current source sets the current that flows into the base of the triode in the frequency selection amplifier, making it work in the near-conduction state, such that when the positive half of the signal that has an average of 0 flows in, the amplifier is turned on and the signal is amplified. In contrast, when the negative half of the signal flows in, the amplifier is turned off, such that looking at the wave that comes out of the amplifier, the high frequency component, the carrier wave, is cut off half. Then the signal passes through an RC filter, which further smooths the signal. This smoothen signal has little carrier wave component in it, ready to be fed to a comparator for digitization. Overall, the bandwidth of this envelope detector is \hl{sss}, the power that supplies it is \hl{aa}, and the gain it multiplies to the input signal is \hl{sss}, as compared to \hl{aa, bb, cc}, respectively, when using a normal envelope detector. Considering our energy budget on \vitag, this amount of saving is significant. 

We illustrate the signal at the input port, at the output port of a traditional envelope detector and at the output port of our low-power envelope detector in Fig.~\ref{fig:sysdiagram} (a). It shows that compared to the output of a traditional detector, the output of our detector is smoother, while having a higher gain. We will see in the following section that the smoother version of the signal is easier to detect using our comparison decoder under the Manchester coding assumption.

\subsubsection{Decoding on an Ultra-Low-Power Device}

Challenges:
\begin{Itemize}
\item Demodulating and decoding the high throughput LED-transmitted data is power consuming. 
\item Transmitting with the LCD at a high toggling frequency consumes even more power than the receiver.
\end{Itemize}

Solution principles:
\begin{Itemize}
\item Use analog components as many as possible (to avoid analog-to-digital converters (ADCs)) and avoid complicated digital signal processing on the mobile end. 
\item Recycle energy spared by the LCD at every toggle.
\end{Itemize}

The output of the envelope detector produces a smoothen wave, yet it is still analog, with continuous values. In principle, a receiver with an ADC can distinguish between the two signal levels by processing the digital samples. Specifically, say we have two signal with different voltages, $V_0$ and $V_1$, $V_0 > V_1$, where $V_0$ and $V_1$ correspond to the power levels for the zero and one bits. To distinguish between then, the receiver would first compute a threshold value. If the duty cycle of the signal is $50\%$, and probabilities of the occurrence of zeros and ones are equal, then the threshold is the average of the two power levels. When the received signal is greater than this threshold, we conclude that the received signal is $V_1$; otherwise, we conclude that the received signal is $V_0$.

Since we choose to eliminate the need for a full ADC in order to reduce power, the receiver is supposed to imitate this operation using analog hardware. This design, though, is slightly different from a conventional ADC, in favor of Manchester coding we use (see~\ref{subsubsec:clockoffset}). The Manchester-encoded signal uses edges to denote bits. Specifically, an \hl{up} edge denotes one, and a \hl{down} edge denotes zero. To achieve consent with this pattern, we design a comparator that detects changes of the voltage. First, using a resister and a capacitor, the comparator sets a time constant that features its detection delay that corresponds to the input data rate. The comparator consistently compares the current analog value $V_{now}$ with the signal value at the last bit $V_{previous}$. If $V_{now} > V_{previous}$, the comparator outputs \hl{one}; otherwise, it outputs \hl{zero}, after a time span of the time constant. 

We note that while a traditional design only performs absolute comparison, our design traces the relative changes in the voltage. Further, using a traditional detector would lead to jagged waveform, which would further cause false comparison results at any edge-oriented comparator. Instead, our comparator design is more suitable for Manchester coding, which is widely adopted for preventing long consecutive ones or zeros in a bit stream, in avoidance of picking a threshold value that is subject to drifting. 





\subsection{\vitag\ Transmitter}
The design of our \vitag\ transmitter builds on off-the-shelf Liquid-Crystal Displays (LCD) and retro-reflectors. The LCD and the retro-reflector combined serve as the modulator for the signal generated by an MCU and amplified on the tag. The LCD's energy is spared each modulation cycle is partially recollected by an energy reuse module that saves $50\%$ of the energy that the tag would have wasted otherwise. The amount of energy saved is of significant importance as to lessening the area of the tag. In addition, the LCD requires a voltage high enough to drive it to its fullest capacity, and this high voltage cannot be directly fed by the low voltage the solar cell can provide. We design a voltage boost module that achieves this with low energy consumption. Overall, the design of the \vitag\ transmitter is presented in Fig.~\ref{fig:sysdiagram} (a).

\subsubsection{LCD and Retro-Reflector-based Modulation}
In the \vitag\ design, we use a retro-reflector to backscatter the incoming light and an LCD put on top of the retro-reflector to modulate the light. In our design, we use a \hl{sss $\times$ bbb} retro-reflector. The reflectivity of the retro-reflector is \hl{sss}, and the Field of View (FoV) is \hl{sss}, which effectively signifies to what degree the reflected signal is focused. The LCD we use is sized \hl{aaa}. 

As electromagnetic waves hit the LCD, the LCD lets the light pass through or blocks it depending on the polarization, i.e., the orientation of the liquid-crystal molecules, in the LCD, which is controlled by the voltage added on it. If the applied voltage is large enough, the liquid crystal molecules are almost completely untwisted and the polarization of the incident light is not rotated as it passes through the liquid crystal layer. This light will then be mainly polarized perpendicular to the second filter, and thus be blocked and the pixel will appear black. The highest voltage applied to the LCD that turns it completely black is \hl{6.1V}, and the lowest voltage with which it starts to be polarized is \hl{2.1V}. We are able to flicker it as fast as \hl{500Hz}. We use the fastest rate as the communication data rate on the uplink, making a \hl{www} power consumption of the LCD. Note, that there are other voltage-controlled reflective materials existing that may have higher flicking rate or lower power. Applying one of those in the system might enhance the energy efficiency and the capacity of the system.  

\subsubsection{Energy Reuse}
The LCD has an equivalent capacitance that corresponds to its periodical charging and discharging. In the discharging phase, if the transmitter has a path along which the current can go all the way from the LCD to the ground, then the energy is wasted. In response, we design an energy reuse module that collects the energy in the LCD discharging phase. The design features a DC/DC converter that boosts the voltage from the lowest voltage that triggers the LCD to the highest. The lowest voltage, as mentioned earlier, is \hl{fff}, which is about the voltage the solar cell array can supply. 

In the charging phase, in which the LCD turns to the blocking mode, the DC/DC boosts the voltage the solar cell supplies to the highest voltage the LCD takes in, as illustrated in Fig.~\ref{fig:sysdiagram} (a). This voltage, through switch $T_0$ the MCU sets to open, applies to the LCD. In this phase, switch $T_1$ is set to close, so the voltage on the LCD gets to pump up until it reaches the discharging phase.

In the discharging phase, the MCU sets the switch $T_0$ to close, and alternatively sets the switch on the discharging path of the LCD $T_1$ to open. Since there is a diode that blocks the only path along which the LCD is supposed to discharge to the ground, the current that flows from the discharging LCD does not go straight to the ground, and instead, it flows back to the DC/DC, charging \hl{$C_0$ and $C_1$}, until the voltage reaches a balance between the LCD and the solar cell. 

The two signals that control the on/off state of the switches are generated by an MCU. When one of the two is set to high, the other is set to low, and vice versa, such that there is only one triode of $T_0$ and $T_1$ open at a time, and so the LCD is either in a charging phase or in a discharging phase, without any conflicts. In addition, we need to make sure that the data rate is slower than the rate at which the two signals from the MCU alternate, so that the voltage on the capacitor-equivalent LCD alternates in a balanced manner in a long run, and $C_0$ and $C_1$ will not constantly be charged or discharged. \vitag\ has \hl{250 bps} data rate, which is smaller than \hl{ccc}, the average time used for charging an empty LCD or discharging a full LCD.






\subsection{\reader\ Receiver}

Challenges:
\begin{Itemize}
\item Detecting the retro-reflected signal against same-band interferences with the LED receiver is hard.
\item The LED must handle clock drifts without explicit synchronization between the LED and the mobile device.   
\end{Itemize}

Solution principles:
\begin{Itemize}
\item Design amplifiers that work at an almost cut-off state to further reduce energy consumption.
\item Design a sliding-window multi-symbol match filter algorithm to remedy clock drifts and LCD-caused signal distortions.
\end{Itemize}

\reader\ captures the signal transmitted by \vitag\ at 250 bps data rate modulated by a 1MHz wave with a light sensor. Upon transferring the fluctuations of the light to voltage, the \reader\ receiver demodulates and decodes the data using RF-end analog circuits and an MCU. While there is less power limit on \reader\ than \vitag, which makes the design more flexible than \vitag, the challenges the \reader\ receiver faces are multi-fold. (1) First, the signal that carries useful information sent by \vitag\ is mixed with the \reader-transmitted signal, which is on a 1MHz carrier as well. What's worse is that since the \reader\ receiver is much closer to the \reader\ transmitter than the \vitag\ transmitter, the strength of the \reader-transmitted signal with the reflections of this signal by the surroundings is in the measurement \hl{ss} times greater than the \vitag-transmitted signal on \reader, making it difficult for the \reader receiver to decouple the two components. (2) Second, the signal carried on 1MHz to be sent by the \reader\ transmitter can also leak to the light sensor, which exacerbates the interference on the light sensor. (3) Third, commercial radios that run on 1MHz could also interfere with the signal that carries useful information. (4) Fourth, the noise caused by the movement of humans and other objects around, along with the circuit noise, could be huge, making the voltage output of the light sensor on \reader\ prone to saturating. In the rest of this section, we describe our \reader\ receiver design (Fig.~\ref{fig:sysdiagram} (b)) that addresses all these challenges, and the techniques that finally make the \vitag\ and \reader\ system practical.

\subsubsection{Extracting Backscatter Information from noise}
Compared with background noise and still-existing interference, the signal strength is weak. For \reader\ receiver, the SINR is \hl{dB}. Specifically, the information bits received \hl{at the light sensor (or after the interference cancellation)} is \hl{dB}, and the interference and noise combined are \hl{dB}. What we finally send to the digital circuit to decode should be a much amplified version of the signal after interference cancellation. Therefore, we need to filter out the carrier wave from the signal and amplify it by \hl{dB}. Using a single amplifier though, is not enough, as there is much more potential of introducing self-excitation to the circuit with too large of an amplification, and the noise introduced by a single amplifier tends to be huge. So we have chosen to apply four separate amplifiers that straddle from the RF-end to the baseband, while performing filtering at each amplifier. The detailed design of this part is the following. To extract the useful information from the noisy background, we first apply an amplifier at the RF end that has the with the amplification of \hl{aa}. This amplifier directly follows the light sensor \hl{or the interference cancellation} with a preliminary LC oscillator that filters out part of the channel noise. Subsequently we add a differential amplifier following a transmission line which decouples the transmitted signal from leaking towards to \reader\ transmitter RF end. The amplification of the differential amplifier is \hl{aa}, with a inductor in parallel with a capacitor that picking out the signal from the carrier wave. Upon filtering, the signal is led to a third amplifier with the amplification of \hl{vv}. The third amplifier is also simultaneously performing filtering, which further picks out a purer signal wave. What follows is the fourth amplifier with feedback and an LC filter. The use of this amplifier is to further increase the signal gain and filter the residual RF-band noise, while bringing the circuit farther from the self-excitation state. After the four levels of amplification, the information signal strength is boosted to \hl{dB}, whereas the background noise is \hl{dB}. And this signal is sent to a envelope detector, which performs regular detection and picks out the baseband signal from that on the 1MHz carrier. 

Overall, this part gives amplification of \hl{dB} on the signal, and achieves \hl{sdd} reduction in the noise. 

\subsubsection{Decoding in the Presence of Clock Offsets}
\label{subsubsec:clockoffset}
Traditionally, the following approaches have been used to extract the timing information from the signal and perform the decoding thereafter.
\begin{Itemize}
\item Peak (edge) detection-based algorithms are ones where samples are taken differentials, and so the extreme (discontinuous) points in the signal are found which denote the clock beats. However, as shown in Fig.~\ref{fig:dynamicRange}, the signal received has a huge dynamic range. If the signal appears to be the case in (a), (b) or (c), the peak approach will fail, as the peak detected will always be ahead of or behind the actual one. In other cases, the edge approach will fail, as the edge is not clearly identified. 
\item Averaging-based algorithms are ones where samples of the signal are averaged to generate a threshold, and samples above this threshold denote ones and below denote zeros. However, as shown in Fig.~\ref{fig:dynamicRange} (e), when the average value of the signal within a packet is drifting, which may happen for the reasons explained earlier, this approach will likely fail. While one could identify a trend for the change in the average value, it is hard to accurately do so in practice. The reason for this is that as the average value is changing in a coherent way, a wrong prediction of the average value will cause severe errors in the process of decoding.
\item Multi-symbol correlation algorithm uses a stream of symbols to represent one bit, and does correlation on the receiver side to decode the bit by finding the peak of the correlation result. The algorithm can pinpoint the clock and hence decode the signal in a low SNR situation, but it is not suitable for low symbol-rate channels like the uplink in our case. 
\item One-symbol match filter tries to match the wave form of the signal and detects the convolution peaks to determine the accurate timing. However, due to the rough equivalence of the LCD on the tag side that shapes a bit and a capacitor, the basic wave form tends to be sawtooth, as shown in Fig.~\ref{fig:dynamicRange} (d) when there is no top or bottom truncation. Further, as the bits are encoded in Manchester code, the rising edge and the falling edge are not necessarily symmetric in time. A typical example is three chips that contain one high-volt chip followed by two low-volt chips, in which case the correlation peak will be skewed, compared to the case where the voltage is high for one chip and low for the next. Therefore, the timing will be biased.
\end{Itemize}

However, decoding on \reader\ is challenging, due to the following reasons: (1) First, the clock information is hard to extract from the received signal. This in part is due to the fact that the start of a frame is hard to accurately identify; this introduces time deviation to \reader\ receiver. Also, there is a frequency offset associated with the clock on the tag that helps generate backscatter signals directionally sent to the reader. On top of these, the clock is subject to drifts. (2) Second, when operating in a network of tags and readers, a tag is likely to receive signals from other readers (although it's designated reader is not transmitting because of the half-duplex mode the system is working in). These signals are 10kHz bit streams sent on a 1MHz carrier. Therefore, when performing demodulation, the 10kHz interference will likely mix with the \hl{125bps} signal of our interest. (3) Compared to the 10kHz interference, what is harder to get rid of from the signal of interest is the noise caused by body movements, the fluctuation in the household electric power supply and its harmonic waves, and changes in environmental brightness that are embedded in the reader-transmitted signal. This set of interference is of low frequencies (humans do not move much faster than 125Hz, so does environmental brightness). Consequently, they mix with the signal transmitted by the tag after preliminary filtering, bringing ever-changing offsets to the signal of interests.

We develop a novel approach to decoding the signal in Manchester code that has a large dynamic range and is saturated with the noise that scatters at about the same frequency. The approach extends the one-symbol match filter to that with an addition regarding clock adjustment using a multi-symbol match filter. The basic idea is to avoid the biased timing caused by skewed correlation peaks that happen in the one-symbol match filter case, by matching all possible patterns of the wave form the Manchester-encoded signal has and accordingly adjusting the local clock frequency in every bit period. To begin with, the algorithm first detects the preamble of a packet using standard correlation, where the preamble is different from any possible bit patterns in the payload. Upon finding the start of a packet, the algorithm estimates the length of a bit first with the knowledge the clock on \vitag that has a known frequency yet subject to drifting. Then the algorithm iteratively does the following two things:
\begin{Itemize} 
\item As every bit is Manchester-encoded, there are two chips within one bit period. A bit-period of a square wave that contains a high volt chip and a low volt chip (not necessarily in this order) correlates against the first three bit-periods of the signal. Based on the difference in value between the first half and the last half within each of the three bit periods, namely, the correlation result within each bit, the algorithm knows what these three bits are among all eight possibilities.
\item Then the algorithm adjusts the clock estimation by correlating the original three bit-periods of the signal against the corresponding one out of the eight patterns that associate with the eight possible wave forms. Ideally, the correlation yields a peak in the middle of the three bits. However, due to the time variance with the start of the packet and the frequency deviation between the reader clock and the tag clock, the peak of the correlation result does not necessarily align with the ideal peak. To bound the clock estimation error along the bits in a packet, we perform linear regression with the estimate of the beginning of the packet and the observations of the bit boundary to get the  estimated beginning of the next bit. With this estimate, the algorithm moves the three-bit window one bit next, and jumps back to perform step one, until reaching the end of the packet. This time recovery algorithm designed specifically for our coding and modulation bounds the error from propagating as the decoding proceeds, as described in the following lemma, for which we give a proof in Appendix.
\end{Itemize}

\begin{lemma}
The time recovery renders the clock estimation error's convergence to zero if a packet contains infinite number of bits. 
\label{lem:lemma1}
\end{lemma}


We note that the reason we choose three-bit period of time as a correlation unit is because three bits are the least number of bit periods that contain all possible wave forms when the signal is Manchester-encoded and LCD capacitor-filtered. We prove this conclusion in~\ref{sec:app}.

Following the bit recovery, \reader\ checks the correctness of the bits received using CRC8 \hl{citation}. The polynomial used is $x^8 + x^2 + x + 1$.

Decoding is taken care of by an MCU. Specifically, we are using \hl{Cortex xxxx} to do that. It has a CPU frequency of \hl{sss} and a \hl{sss} memory, hence good for performing complex algorithms and dealing with fast streaming data. 


% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/divide.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf Signal Captured by the LED Light Sensor \hl{replace with a system block diagram!!}} \hl{integrates both mmm in a single design. It can operate using both RFID and TV transmissions}.}
% \label{fig:capture}
% \vskip -0.05in
% \end{figure}





\begin{figure*}[!t]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{ccccc}
\epsfig{file=fig/waveform1-eps-converted-to.pdf, width=0.4\columnwidth} & \epsfig{file=fig/waveform2-eps-converted-to.pdf, width=0.4\columnwidth} & \epsfig{file=fig/waveform3-eps-converted-to.pdf, width=0.4\columnwidth} & \epsfig{file=fig/waveform4-eps-converted-to.pdf, width=0.4\columnwidth} & \epsfig{file=fig/waveform5-eps-converted-to.pdf, width=0.4\columnwidth}\\
{(a) Normal} & {(b) Up-truncated} & {(c) Down-truncated} & {(d) Up and Down-truncated} & {(e) Average-drifted}\\
\end{tabular}
}
\vskip -0.1in
\caption{\footnotesize{\bf Varying Wave patterns.} Blah Blah.}
\label{fig:dynamicRange}
\vspace{-1em}
\end{figure*}

==> ViTag_2.tex <==
\section{\retro\ Design}

% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/corr-bd.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf System Diagram} (a) \vitag\ and (b) Modified LED.}
% \label{fig:sysdiagram}
% \vskip -0.05in
% \end{figure}

\begin{figure*}[!t]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{cc}
\epsfig{file=../illustrations/tag.eps, width=2\columnwidth} \\ {(a) \vitag\ Block Diagram}\\
\epsfig{file=../illustrations/reader.eps, width=2\columnwidth} \\ {(b) LED Block Diagram}\\
\end{tabular}
}
\vskip -0.1in
\caption{\footnotesize{\bf System Diagram.} Blah Blah.}
\label{fig:sysdiagram}
\vspace{-1em}
\end{figure*}

\retro\ is a new form of communication in which battery-free \vitag\/s can communicate with LEDs without any additional infrastructure. Harvesting LED light energy, a \vitag\ reflects visible light signals to communicate. Because of the ubiquitous deployment of illuminating LEDs, building such a system will enable ubiquitous communications at an unprecedented scale. It will also enhance the security of current RFID systems as it limits the uplink signal exposure to line-of-sight, and the use of retro-reflectors will further focus the signal to an even thiner area, leaving less chance for the hidden attackers and sniffers to temper the system.

Designing such a system, however, faces several challenges, which we will break down in the following subsections, and we describe how our design address these challenges.


%Designing such tags, however, is challenging for four reasons: First, the visible light that carries data is interleaving with intensive interference, such as radios operating at the same frequency, and the light emitted from the LEDs that also carries data and its reflections from surrounding walls, thus making an interference-intensive receiving condition for both \vitag\ and \reader. Second, the signal is exposed to noise, such as the existing environmental lights that is subject to constant changing, human-body-movement-caused noise, and the noise caused by the hardware system itself. Third, to emit modulated light from \vitag\ and make it detectable by \reader\ on a battery-free tag is challenging in that modulating signals on visible light bands is power-consuming with respect to the goal of being battery-free. Finally, to integrate the system to off-the-shelf LED lights while keeping the brightness of the lights constant is challenging. In the rest of this section and the next section, we describe how our design addresses the above challenges.




\subsection{Overview}
Fig.~\ref{fig:sysdiagram} (a) shows a block diagram of our \vitag\ design. It consists of a transmitter, a receiver, an MCU and a harvester. The transmitter and receiver communicate by modulated backscattering of visible light signals, and the harvester absorbs energy from visible lights to power the device. Further, they operate independently of each other. The receiver immediately awakes the MCU by rising the tag voltage to a certain value and enabling the analog circuit to start receiving as it detects a data packet coming in. The MCU then shuts down the analog circuit and powers up the transmitting circuit. The receiving circuit and the transmitting circuit work alternately to save energy. Alongside the communication modules is the energy harvester, which consists of a number of solar cells that transfer visible light energy into electric energy. The harvester sets the upper bound of the power \vitag\ can take on, thus posing a strict constraint to the design of each component on the tag.

Fig.~\ref{fig:sysdiagram} (b) shows a block diagram of our \reader\ design. The major part of it is an LED bulb that emits fast-fluctuating light human eyes cannot detect flickering in. \reader\ builds on off-the-shelf LEDs and makes minor modifications on them. It consists of a transmitter, a receiver and an MCU. The transmitter encodes and modulates the data, feeding the data to the LED for transmission, while keeping the LED not flickering and with dimming support. The transmitter also takes the goal of making \vitag\ battery-free in mind, emitting lights with data such that \vitag\ can demodulate and decode the data at a low energy cost. The receiver deals with the light backscattered from \vitag, and also cancels noise and interference as much as possible. The MCU processes the data transmitted from \vitag.

Next, we describe our design of the transmitter and receiver on the \vitag\ and LED in more detail.





\subsection{\reader\ Transmitter}
\label{subsec:LEDtrans}

As shown in Fig.~\ref{fig:sysdiagram} (b), the transmitter on \reader\ is composed of a crystal oscillator that runs at 1MHz\footnote{The fastest flickering rate of our LED is 1MHz}, and an MCU followed by two amplifiers. The MCU-generated bits toggle the crystal oscillator to OOK the signal with Manchester encoding. The modulated signal will then be amplified and fed to a LED. To make sure the brightness of the LED does not pose a difference between the transmitting and not transmitting state, we add a DC component to the signal. The magnitude of the DC component is adaptable so that we can dim the brightness of the LED emission. In addition to the dimming support, flickers are avoided in \reader\ transmitter. We use 10kHz as the data rate, which far exceeds the frequency (200 Hz) below which human eyes will feel of fluctuations, which could disturbing and unacceptable. 


% We illustrate a typical packet the LED transmits in Fig.~\ref{fig:commdiagram}.

% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/layout2.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf An LED-transmitted Packet} \hl{blah}.}
% \label{fig:commdiagram}
% \vskip -0.05in
% \end{figure}

% We note the following about our design: Firstly, we use a white-colored LED, which emits electromagnetic waves of wavelengths between 380 and 780 nm. The highest flickering frequency of the LED with full on/off transitioning is 1MHz, and we are exploiting the flickering rate to its fullest, in order to leave room for downlink data rate as high as possible. 

% Secondly, different components in the transmitter on the reader side require different voltage supply. We are using two DC/DCs to boost the voltage for the switch and the amplifiers. Specifically, the voltage used for supply the crystal oscillator, the amplifiers for the MCU-output signals and the switch is 5V, and the voltage for the amplifiers for the RF signals is 12V. 

% Finally, the 1MHz frequency, as mentioned earlier, is used because of the full flickering capability we would like to draw from the LED. However, around this frequency with a bandwidth on the order of 100kHz, there are commercial radios using AM modulation. For example, there are radios from 540 through 1610 kHz with 10 kHz spacing in America. Another form is situated at a similar spectrum spanning from 531 to 1611 kHz with 9 kHz spacing. There are also other interferences, which we address in later sections.





\subsection{\vitag\ Receiver}

\begin{tcolorbox}
\vskip 0.05in\noindent{\bf Challenge:} It is power consuming to Demodulate and decode the high throughput LED-transmitted data.
\vskip 0.05in\noindent{\bf Solution Principle:} Use analog components as many as possible (to avoid ADCs) and avoid complicated digital signal processing on the mobile end. Also, design amplifiers that work at an almost-cut-off state to save energy cost.
\end{tcolorbox}

Following the flow of the signal, we describe the design of our \vitag\ receiver. We first use a light sensor\footnote{A normal light sensor has a bandwidth of over 1GHz} that captures the visible light. The captured signals then go through filters, detectors/demodulators, and another feedback amplifier before being sent to a comparator be digitized. We only use analog elements and a low-power microcontroller for receiving, and design modules that set the amplifiers to work at an almost-cut-off state, where the energy consumption is extremely low. The block diagram of the receiver is presented in Fig.~\ref{fig:sysdiagram} (a).

\subsubsection{Extracting Information from the Visible Light}
\reader\ transmitted signals are captured with a light sensor. The light sensor has an equivalent capacitance, which, with an inductor parallel to it, performs preliminary front-end filtering. Next, two amplifiers successively amplify the RF signal while avoiding auto-excitation using a feedback mechanism. Upon preliminary filtering and amplification, the signal is ready for demodulation. Avoiding the downside of a conventional envelope detector on high power consumption, our demodulator contains a constant current source, a diode, and a frequency selection amplifier. The constant current source sets the current that flows into the base of the triode in the frequency selection amplifier, making it work at an almost-cut-off state, such that the amplifier is turned on and the signal is amplified when the positive half of the signal that has an average of 0 flows in. On the other hand, when the negative half of the signal flows in, the amplifier is turned off. This process essentially demodulates the signal from the 1MHz carrier. Finally, the signal passes through an RC filter, which further smooths the signal, ready to be fed to a comparator for digitization. Overall, our demodulator saves more energy than a conventional envelope detector because of the low-energy working region ours works in. We also note that the output of our demodulator is smoother, while having a higher gain than a traditional envelope detector, which is favorable in the energy-constrained decoding phase.

\subsubsection{Decoding on an Ultra-Low-Power Device}

While the output of the envelope detector is a smooth wave, it is still analog with continuous values. In principle, a receiver with an ADC can distinguish between the two signal levels by processing the digital samples. Specifically, say we have two signals with different voltages, $V_0$ and $V_1$, $V_0 > V_1$, where $V_0$ and $V_1$ correspond to the power levels for the zero and one bits. To distinguish between them, the receiver would first compute a threshold value. If the duty cycle of the signal is $50\%$, and odds of the occurrence of zeros and ones are equal, then the threshold is the average of the two power levels. If the received signal is greater than this threshold, we conclude that the received signal is $V_1$; else, we conclude that the received signal is $V_0$.

Since we seek to eliminate the need for a full ADC in order to reduce power, the receiver should imitate this operation using analog hardware. In favor of Manchester coding we use (see~\ref{subsec:LEDtrans}), the goal of our design, however, is different from a typical ADC. The Manchester-encoded signal uses edges to denote bits. Specifically, an up edge denotes one, and a down edge denotes zero. To align with this pattern, we design a comparator that detects changes of the voltage. First, using a resister and a capacitor, the comparator sets a time constant that features its detection delay that corresponds to the input data rate. The comparator consistently compares the current analog value $V_{now}$ with the signal value at the last bit $V_{previous}$. If $V_{now} > V_{previous}$, the comparator outputs $1$; otherwise, it outputs $0$. We note that while a traditional design only performs absolute comparison, our design traces the relative changes in the voltage. Further, using a traditional detector would lead to jagged waveform, which would further cause false comparison results at any edge-based comparator. Instead, our comparator design is more suitable for Manchester coding, which is widely adopted for preventing long consecutive $1$s or $0$s in a bit stream, in avoidance of picking a threshold value that would suffer from drifting. 

THe microcontroller then works to check the correctness of the packet. In the receiving phase, microcontroller consumes $120\mu A$.





\subsection{\vitag\ Transmitter}
\label{subsec:tagtrans}

\begin{tcolorbox}
\vskip 0.05in\noindent{\bf Challenge:} Transmitting with the LCD at a high toggling frequency consumes even more power than the receiver.
\vskip 0.05in\noindent{\bf Solution Principle:} Recycle energy spared by the LCD at every toggle; And use an RC oscillator instead of the crystal oscillator used in the receiving phase.
\end{tcolorbox}


Our \vitag\ transmitter transmits by passively backscattering the incoming light. The core of the transmitter is the combination of an LCD and a retro-reflector that serves as a modulator. To conserve energy, we design an energy reuse module that, in every modulation cycle, recollects $50\%$ of the energy that would have been wasted by the LCD without such a module. To further save energy, instead of using power-demanding crystal oscillators, we use a simple RC oscillator to generate control signals to toggle the LCD. While the RC oscillator does have worse clock stability and a lower frequency, we design modules that address these issues in~\ref{subsec:LEDreceiver}. Finally, the LCD requires a voltage high enough to drive it to its fullest capacity, and this high voltage cannot be directly fed by the low voltage the solar cell can provide. We design a voltage boosting module that achieves this. The overall design of the \vitag\ transmitter is presented in Fig.~\ref{fig:sysdiagram} (a). We now break down the design into the following key points.

\subsubsection{Modulating the Retro-Reflector with an LCD}
To avoid actively generating light signals, which may cost way more power than affordable on a battery-free \vitag, we instead take the advantage of retro-reflectors that passively bounce the incoming light back. As described in Section~\ref{sec:background}, the retro-reflector has the merit that it can directionally bounce the light at a direction same as the one the light arrives at. To modulate the light, we cover the retro-reflector with an LCD. When at work, as electromagnetic waves hit the LCD, the LCD lets the light pass through or blocks it depending on the polarization, i.e., the orientation of the liquid-crystal molecules, in the LCD, which is controlled by the voltage added on it. If the applied voltage is large enough, the pixels will appear black. The highest voltage applied to our LCD that turns it completely black is $6.1V$, and the lowest voltage with which it starts to be polarized is $2.1V$. We are able to flicker it as fast as $1kHz$, which also is our highest data rate on the uplink. Note, that there are other voltage-controlled reflective materials existing that may have higher flicking rate or lower power. Applying one of those in the system might enhance the energy efficiency and the capacity of the system.  

\subsubsection{Energy Reuse}
The current that feeds the LCD which has an equivalent capacitance of $9nF$ would be wasted to the ground when the LCD discharges. However, we found that by recollecting this portion of the current in the LCD discharging phase, $50\%$ of the energy could be saved. In response, we designed an energy reuse module, illustrated in Fig.~\ref{fig:energyreuse}, that features a DC/DC converter that boosts the voltage from the lowest voltage that triggers the LCD to the highest. The lowest voltage, as mentioned earlier, is $2.1V$, which is about the voltage the solar cell array can supply. 

In the charging phase, in which the LCD turns to the blocking mode, the DC/DC boosts the voltage the solar cell supplies to one the LCD reaches its full capacity at. This voltage effectively applies to the LCD when the MCU sets $T_0$ to open, while $T_1$ is set to close. The voltage on the LCD pumps up to $6.1V$ and stays until the discharging phase.

In the discharging phase, the MCU sets $T_0$ to close, and $T_1$ to open. Since there is a diode that blocks the only path along which the LCD could discharge towards the ground, the current that flows from the discharging LCD does not go straight to the ground; Instead, it flows back to the DC/DC, charging $C_0$ and $C_1$, until the voltage on the LCD equals to that on the solar cell. 

We note two things about our design. First, the two signals that control the on/off state of the switches are generated by an MCU. When one of the two is set to high, the other is set to low, and vice versa, As a result, there is only one triode between $T_0$ and $T_1$ open at a time, so the LCD is either in a charging phase or in a discharging phase, with no conflict. Second, we always make sure that the data rate is slower than the rate at which the two signals from the MCU alternate, so that the LCD alternates in a balanced manner without saturation in a long run, i.e., $C_0$ and $C_1$ will not constantly be charged or discharged. In real world settings, fortunately, the \vitag\ has up to $1kbps$ data rate, which is much smaller than the average time used for charging an empty LCD or discharging a full LCD.

\begin{figure}[!t]
\vskip -0.03in
  \centering
      {
        \epsfig{file=../illustrations/EnergyReuseCircuits.eps, width=0.6\columnwidth}
      }
\caption{{\bf Our Energy Reuse Module} \hl{blah}.}
\label{fig:energyreuse}
\vskip -0.05in
\end{figure}





\subsection{\reader\ Receiver}
\label{subsec:LEDreceiver}

\begin{tcolorbox}
\vskip 0.05in\noindent{\bf Challenge:} The LED receiver must handle time offsets caused by the \vitag's RC-based clock with low oscillating frequency, and has to detect the retro-reflected signal which is 3 orders of magnitude weaker than interfering LED transmissions.   
\vskip 0.05in\noindent{\bf Solution Principle:} Design a sliding-window multi-symbol match filter algorithm to remedy clock drifts and LCD-caused signal distortions.
\end{tcolorbox}

The \reader\ captures the signal transmitted by \vitag\ at an up to $1kbs$ data rate on a 1MHz carrier. Upon transferring the light signal to voltage, the \reader\ receiver demodulates and decodes the data using RF-end analog circuits and the same microcontroller the \reader\ transmitter uses. While there is less power limit on \reader\ than \vitag, the \reader\ receiver design still faces multi-fold challenges. (1) First, the signal sent by the \vitag\ is mixed with the \reader-transmitted signal, which, too, is on a 1MHz carrier. Since the \reader\ receiver is much closer to the \reader\ transmitter than the \vitag\ transmitter, the strength of the \reader-transmitted signal with the reflections of this signal by the surroundings 3 orders of magnitude greater than the \vitag-transmitted signal on \reader. As we measure, the typical voltage of the received signal is on the order of magnitude of $mV$, while the voltage supply for the LED receiver is $8V$. (2) Second, the signal carried on 1MHz to be sent by the \reader\ transmitter can also leak to the light sensor, which exacerbates the interference. (3) Third, commercial radios that run on 1MHz could also interfere with the signal that carries useful information. (4) Fourth, the noise caused by the movement of humans and other objects around could be huge. The voltage output of the light sensor on the \reader\ is therefore prone to saturating. (5) On top of these, as we noted in~\ref{subsec:tagtrans}, the received signal suffers from timing offsets caused by the low-cost low-frequency clock on the \vitag. In the rest of this section, we describe our \reader\ receiver design (Fig.~\ref{fig:sysdiagram} (b)) that addresses these challenges.

\subsubsection{Extracting Backscatter Information from noise}
Since the signal to interference ratio is extremely low (~mV against ~V), we have to amplify the received signal more than $1000$ times in magnitude. Using a single amplifier though, is not feasible, as the potential of introducing self-excitation to the circuit with a huge amplification is high, and the noise introduced by a single amplifier tends to be unacceptable. So we apply five successive amplifiers instead. The detailed design is the following. To extract the useful information from the noisy background, we first apply an amplifier at the RF end. This amplifier directly follows the light sensor with an LC filter that performs preliminary band-pass filtering. Subsequently, we add a differential amplifier following a transmission line which decouples the transmitted signal from leaking towards the RF end. There is an impedance matching module between the light sensor filter and the transmission line. Now, the center frequency of the differential amplifier is $1MHz$ with the help of an LC module, and its gain is controlled by the microcontroller. The third and fourth amplifiers are also with LC modules that perform further RF-band filtering. The fourth amplifier is with feedback mechanism. The use of this amplifier is to further increase the signal gain and filter the residual RF-band noise, while dragging the circuit state farther from self-excitation. After the amplifications, this signal is sent to an envelope detector, which performs regular demodulation that picks out the baseband signal from the $1MHz$ carrier. Finally, the same comparator used on the \vitag\ is used to digitize the Manchester-encoded signal.  


\subsubsection{Decoding in the Presence of Clock Offsets}
\label{subsubsec:clockoffset}

Traditionally, the following approaches have been used to extract the timing information from the signal and perform the decoding thereafter.

\vskip 0.05in\noindent{\bf Peak (edge) detection-based algorithms} are ones where samples are taken differentials, and so the extreme (discontinuous) points in the signal are found which denote the clock beats. However, as shown in Fig.~\ref{fig:dynamicRange}, the signal received has a huge dynamic range. If the signal appears to be the case in (a), (b) or (c), the peak approach will fail, as the peak detected will always be ahead of or behind the actual one. In other cases, the edge approach will fail, as the edge is not clearly identified. 
\vskip 0.05in\noindent{\bf Averaging-based algorithms} are ones where samples of the signal are averaged to generate a threshold, and samples above this threshold denote ones and below denote zeros. However, as shown in Fig.~\ref{fig:dynamicRange} (e), when the average value of the signal within a packet is drifting, which may happen for the reasons explained earlier, this approach will likely fail. While one could identify a trend for the change in the average value, it is hard to accurately do so in practice. The reason for this is that as the average value is changing in a coherent way, a wrong prediction of the average value will cause severe errors in the process of decoding.
\vskip 0.05in\noindent{\bf Multi-symbol correlation algorithms} use a string of symbols to represent one bit, and does correlation on the receiver side to decode the bit by finding the peak of the correlation result. The algorithm can pinpoint the clock and hence decode the signal in a low SNR situation, but it is not suitable for low symbol-rate channels like the uplink in our case. 
\vskip 0.05in\noindent{\bf One-symbol match filter algorithms} try to match the wave form of the signal and detects the convolution peaks to determine the accurate timing. However, due to the rough equivalence of the LCD on the tag side that shapes a bit and a capacitor, the basic wave form tends to be sawtooth, as shown in Fig.~\ref{fig:dynamicRange} (d) when there is no top or bottom truncation. Further, as the bits are encoded in Manchester code, the rising edge and the falling edge are not necessarily symmetric in time. A typical example is three chips that contain one high-volt chip followed by two low-volt chips, in which case the correlation peak will be skewed, compared to the case where the voltage is high for one chip and low for the next. Therefore, the timing will be biased.

We develop a novel algorithm to decode the signal encoded with Manchester code that has a large dynamic range. We term it a sliding-window multi-symbol match filter algorithm. The approach extends the one-symbol match filter to that with an addition regarding clock adjustment using a multi-symbol match filter. The basic idea is to avoid the biased timing caused by skewed correlation peaks that happen in the one-symbol match filter case, by matching all possible patterns of the wave form the Manchester-encoded signal appears to have, and iteratively adjusting the local clock by every bit period. To begin with, the algorithm exploits standard correlation to detect the preamble of a packet, using the fact that the preamble is different from any possible bit patterns in the payload. Upon finding the start of a packet, the algorithm estimates the length of a bit first using the knowledge of the \vitag\ clock that has a known frequency yet subject to offsets. Then the algorithm iteratively does the following two things:

\vskip 0.05in\noindent{\bf Step 1: Wave Form Recognition.} As every bit is Manchester-encoded, one bit contains two chips. A bit-period of a square wave that contains a high volt chip and a low volt chip (not necessarily in this order) correlates against the first three bit-periods of the signal. After this, the algorithm knows what these three bits are out of eight possible wave forms.

\vskip 0.05in\noindent{\bf Step 2: Local Time Recovery.} Then the algorithm adjusts the clock estimation by correlating the three bits from the raw signal against the corresponding gold pattern from the eight patterns. Ideally, the correlation yields a peak in the middle of the three bits. However, due to the time variance with the start of the packet and the frequency deviation between the reader clock and the tag clock, the peak of the correlation result does not necessarily align with the ideal peak. To bound the clock estimation error along the bits in a packet, we perform linear regression $t=k\dot s+s_0$ to estimate the timing of the next three bits, using the estimate of the beginning of the packet as $s_0$ and the estimate of the current three bits and their timing as the training data ${s,t}$. Every round $k$ is re-estimated, and then the algorithm moves the three-bit window one bit forward, and jumps back to perform step one, until reaching the end of the packet. This time recovery algorithm designed specifically for our coding and modulation bounds the error on $k$ from propagating as the decoding proceeds. We formally describe this in the following lemma, for which we give a proof in Appendix.


\begin{lemma}
The time recovery renders the clock estimation error's convergence to zero if a packet contains infinite number of bits. 
\label{lem:lemma1}
\end{lemma}


We note that we choose a three-bit time span as a correlation unit because three bits are the smallest number of bits that contain all possible wave forms when the signal is Manchester-encoded and LCD capacitor-filtered.

Following the local time recovery and decoding, \reader\ checks the correctness of the bits received using CRC8. The polynomial used is $x^8 + x^2 + x + 1$.


% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/divide.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf Signal Captured by the LED Light Sensor \hl{replace with a system block diagram!!}} \hl{integrates both mmm in a single design. It can operate using both RFID and TV transmissions}.}
% \label{fig:capture}
% \vskip -0.05in
% \end{figure}





\begin{figure*}[!t]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{ccccc}
\epsfig{file=../illustrations/waveform1.eps, width=0.35\columnwidth} & \epsfig{file=../illustrations/waveform2.eps, width=0.35\columnwidth} & \epsfig{file=../illustrations/waveform3.eps, width=0.35\columnwidth} & \epsfig{file=../illustrations/waveform4.eps, width=0.35\columnwidth} & \epsfig{file=../illustrations/waveform5.eps, width=0.35\columnwidth}\\
{(a) Normal} & {(b) Up-truncated} & {(c) Down-truncated} & {(d) Up and Down-truncated} & {(e) Average-drifted}\\
\end{tabular}
}
\vskip -0.1in
\caption{\footnotesize{\bf Varying Wave patterns.} Blah Blah.}
\label{fig:dynamicRange}
\vspace{-1em}
\end{figure*}

==> background.tex <==
\section{Preliminaries}
\label{sec:background}

\begin{figure*}[!t]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{cccc}
\epsfig{file=fig/mrr1-eps-converted-to.pdf, width=0.5\columnwidth} &
\epsfig{file=fig/mrr2-eps-converted-to.pdf, width=0.5\columnwidth} & 
\epsfig{file=fig/mrr3-eps-converted-to.pdf, width=0.5\columnwidth} & 
\epsfig{file=fig/mrr4-eps-converted-to.pdf, width=0.5\columnwidth} \\
{(a) Same Direction} & {(b) Different Directions} & {(c) With LCD on} & {(d) Retro-reflector Principle}\\
\end{tabular}
}
\vskip -0.1in
\caption{\footnotesize{\bf Illustration of the Retro-reflector.} Blah Blah.}
\label{fig:retrolcd}
\vspace{-1em}
\end{figure*}



In this section, we introduce a few concepts which are used throughout the paper. 

%In principle, \vitag\ is a general technique that can leverage visible light signals to do full-stack secure communications between an array of powered sources and battery-free backscatter devices. In this paper, we demonstrate this feasibility with an RFID-based application, and show that it is better than the existing RFID technology in several critical aspects. 

\paragraph{Visible Light Communication} 
Visible lights are electromagnetic waves that span frequencies roughly from $400$ to $800 THz$. Commonly, white LEDs are used for illumination. The instantaneous On/Off feature turns LEDs into effective transmitters for visible light communication (VLC). Specifically, information bits can be embedded on the light by modulating the on/off state of the LED with on-off keying (OOK) or variable pulse-position modulation (VPPM) \cite{standard}. To receive such signals, while in some cases a cell phone camera or a digital camera will be sufficient \hl{need citations, ipsn14 and mobicom14}, photodiodes are generally used, because phone cameras can only achieve around 0.25MHz sampling rate~\cite{camera1} (in other words, low data rate), whereas photodiodes have generally higher bandwidth up to 0.5GHz~\cite{pdsheet}. Moreover, compared with a phone camera, the SNR of the photodiode is orders of magnitude higher at the same distance \hl{ipsn14}. 

%A typical way to generate white lights is to use a phosphor material to convert monochromatic lights from blue or ultraviolet to broad-band white lights, where the color of the monochromatic light depends on the band gap energy of the materials forming the p-n junction in the LED. 

%Visible lights bring safety advantages over communication waves of other common frequencies, because human eyes are much more sensitive to the strength of visible lights than the invisible TV, Wi-FI and RFID transmissions. With the LED dimming support~\cite{dimming}, a person can turn down the light if she feels of a too high brightness. In addition, radios waves at some certain frequencies are likely to hard human organs, especially to pregnant women and kids~\cite{rfidharm}, while the visible light are not.

%There are two primary ways of producing white LEDs. One is to use individual LEDs that emit three primary colors --- red, green, and blue --- and then mix all the colors to form white light~\cite{ledprin1}. The other is to use a phosphor material to convert monochromatic light from a blue or UV LED to broad-spectrum white light, much in the same way a fluorescent light bulb works~\cite{ledprin2}. In general, the wavelength of the light emitted, and thus its color, depends on the band gap energy of the materials forming the p-n junction. In materials used for LEDs, the electrons and holes recombine by a radiative transition, which produces optical emission, because there are direct band gap with energies corresponding to near-infrared, visible, or near-ultraviolet light. 



\paragraph{Retro-reflector} 
Retro-reflector is a device or surface that operate by returning light back to the light source along the same light direction with a minimum of scattering \hl{cite the wikipage}. Retro-reflectors are widely used on road signs, bicycles, and clothing for road safety. From a microscopic view, a retro-reflector is composed of cells, each of which is a corner cube as shown in \hl{Fig.xx}. When a light beam hits one of the cells, the light is turned around via two adjacent reflections. 

Modulating retro-reflector (MRR) \hl{cite the wikipage} is a system typically consisting of a retro-reflector and a modulator for optical communications. The MRR operates as a passive sources which transmits bits by varying the intensity of the reflected light beam. MRR is widely used in free space communication where the other side is a laser. Existing MRR \hl{cite some papers} is usually with large size, and modulation is commonly achieved with a high-end electroabsorption modulator altering the absorption spectrum by applying an electric field. Consequently, such setting is ill-suited for our scenarios which require a low-cost solution.
 
\paragraph{Liquid-crystal display (LCD)}
LCD is a type of display widely used in portable devices like digital watches and phones. LCDs do not emit light directly; Rather, they use the light properties of liquid crystals that are controlled by the voltage added on them. When the LCD is on, the incoming light is able to pass the LCD and hit the retro-reflector; When the LCD is off, the incoming light is rejected by the LCD. Therefore, LCDs can be used as modulators for MRRs. However, one disadvantage of LCDs are their low refresh rate, e.g., 60 or 75 Hz, which is too low for data communication. Fortunately, we find \textit{LCD shutters} with much higher refresh rate (up to 1KHz \hl{cite}). Fig.~\ref{fig:retrolcd} shows the basic principle of a retro-reflector with an LCD coverage.



==> bg_copy.tex <==
\section{Requirements and Preliminaries}
\label{sec:background}

\subsection{Requirements}

Our goal is to establish a bi-directional communication link using visible lights. As the dual-paradigm nature of VLC over the lighting infrastructure entails that the primary function is illumination and the primary usage scenario is communicating with low power mobile devices or sensor nodes, we have the following two basic requirements behind the goal. 

\noindent\emph{\textbf{Requirement 1:}} Establish a low-power, duplex visible light communication link with a battery-free mobile end that harvests light energy from the illumination LED. 

\noindent\emph{\textbf{Requirement 2:}} Impose no constraints on the actual usage. This implies a practical working range in normal indoor situations, ease of use, and that the size of the device should be small for convenience.

To achieve a duplex visible link, one possibility is to use a symmetric design, that is, using an LED on the mobile device or sensor node to actively emit signals, which are picked up by a light sensor on the lighting LED. Unfortunately, to be able to reach a practical working distance (with the light typically installed on the ceiling) costs prohibitively high energy on the mobile device of a credit card size. Being electromagnetic radio in nature, the light energy attenuates quickly as propagation proceeds~\cite{lightwave}.

One way to extend the communication range is to use directional signals, ideally a laser. However, that would require manual alignment between the light source and the mobile device. 

Another possible way towards more affordable power is to leverage the light from the lighting infrastructure, which is usually of high power. This is similar to the design of passive RFID systems where the tag communicates with the reader by reflecting the incoming radio signal. For instance, we may use a \textit{mirror} to reflect the light from the LED back to a light sensor collocated on the LED. However, a mirror makes highly directional reflection. Such a design would also require carefully orienting the mobile device and violate the practicality requirement. 

Inspired by free space laser communication systems~\cite{mrr}, we use a retro-reflector to meet requirement 2. Below we introduce the retro-reflector and present some favorable properties about retro-reflector materials. 



\subsection{Preliminaries}

\begin{figure}[tb]
    \centering
    \subfigure[Corner Cube Illustration]{
        \includegraphics[width=0.45\columnwidth]{../illustrations/retroreflector.eps} 
        \label{fig:cornercube}
    } \hfill
    \subfigure[Bicycle Retro-reflector]{
        \includegraphics[width=0.45\columnwidth]{1280px-BicycleRetroreflectors.jpg}
        \label{fig:bike-cc}
    } 
     \caption{\label{fig:retro-reflector}Principle of a retro-reflector and sample products.}
%      \vspace{-5mm}
  \end{figure}

\paragraph{Retro-reflector} 
A retro-reflector is a device or surface that, unlike mirrors, reflects light back to its source along the same incoming direction with little scattering~\cite{rr}. 

A retro-reflector can be produced using spherical lens, much like the mechanism of a cat's eye. A more feasible way to obtain retro-reflection is to use a corner reflector, which consists of a set of cubes each with three mutually perpendicular reflective surfaces. The principle of such a retro-reflector is shown in \figref{fig:cornercube}. A large yet relatively thin retroreflector is possible by combining many small corner reflectors, using the standard triangular tiling. Such thin retro-reflectors are widely used on road signs, bicycles, and clothing for safety. \fyi{\figref{fig:bike-cc} shows a flattened retro-reflector seen on bicycles.} \todo{May merge Fig 1 and 2, by removing the current fig 2(d).}


%\begin{figure*}[!th]
%  \begin{center}
%      \subfigure[TX $90\degree$, RX $90\degree$]{
%        \includegraphics[height=0.2\columnwidth]{../illustrations/mrr4.eps}\label{fig:mrr4}
%      } 
%      \hfill
%      \subfigure[TX $45\degree$, RX $45\degree$]{
%        \includegraphics[height=0.2\columnwidth]{../illustrations/mrr1.eps}\label{fig:mrr1}
%      } 
%      \hfill
%      \subfigure[TX $45\degree$, RX $90\degree$]{
%        \includegraphics[height=0.2\columnwidth]{../illustrations/mrr3.eps}\label{fig:mrr3}
%      }
%%      \vspace{-1em}
%      \caption{Optical properties of a retro-reflector fabric, comparing with a white paper and a planar mirror. (a) When the LED is at $90\degree$, and the camera is at $90\degree$, both the retro-reflector and mirror areas are bright. (b) When the LED (TX) is at $45\degree$ arrival of incidence, and the camera (RX) is at $45\degree$, the retro-reflector area (on the right) is bright, the mirror area (in the middle) is dark, and the paper area (on the left) is dark. (c) When the LED is at $45\degree$, and the camera is at $90\degree$, the retro-reflector and the mirror areas are dark, while the paper area is slightly bright due to diffused reflections. \todo{Need to separate the figures without LCD. Make sure the exposure to be the same. Pay attention to the aspect ratio.}}\label{fig:rr-reflection}
%  \end{center}
%%  \vspace{-0.3in}
%\end{figure*}

\iftrue
\begin{figure}[th]
  \begin{center}
      \subfigure[Flash at $90\degree$, Camera at $90\degree$]{
        \includegraphics[width=0.46\columnwidth]{tx90-rx90.jpg}\label{fig:mrr4}
      } 
      \hfill
      \subfigure[Flash at $45\degree$, Camera at $90\degree$]{
        \includegraphics[width=0.45\columnwidth]{tx45-rx90.jpg}\label{fig:mrr3}
      } \\
      \subfigure[Flash at $45\degree$, Camera at $45\degree$]{
        \includegraphics[width=0.45\columnwidth]{tx45-rx45.jpg}\label{fig:mrr1}
      } 
      \hfill \hspace{-1ex}
    \subfigure[Reflection dispersion]{
        \includegraphics[width=0.5\columnwidth]{rr-angle.png}
        \label{fig:rr-angle}
    } 

%      \vspace{-1em}
      \caption{Optical reflection properties of a retro-reflector fabric (Scotchlite from 3M) (right), compared with a white paper (left) and a planar mirror (middle).}\label{fig:rr-reflection}
  \end{center}
%  \vspace{-0.3in}
\end{figure}
\else
\begin{figure}[!th]
  \begin{center}
    \subfigure[Reflection property]{
        \includegraphics[width=0.9\columnwidth]{RR-property-exp.pdf}
        \label{fig:rr-exp}
    } \\
    \subfigure[Reflection property]{
        \includegraphics[width=0.7\columnwidth]{rr-angle.png}
        \label{fig:rr-angle}
    } 

%      \vspace{-1em}
      \caption{Optical properties of a retro-reflector fabric, comparing with a white paper and a planar mirror. \todo{Need to separate the figures without LCD. Make sure the exposure to be the same. Pay attention to the aspect ratio.}}\label{fig:rr-reflection}
  \end{center}
%  \vspace{-0.3in}
\end{figure}
\fi


%      \vspace{-5mm}

We conduct experiments to measure the reflecting properties of our retro-reflector fabric (Scotchlite from 3M~\cite{rrsheet}). We compare it against a plain white paper which features diffusing reflection and a planar mirror that does mirror reflection. We place the three materials side by side and let the light source (a flash light) emit light at different angles while retaining the same distance to the materials. We use a camera to capture reflected light. \figref{fig:rr-reflection} shows the resulting images from experiments conducted in a dark chamber. In the figures, we can see that the retro-reflector fabric is bright as long as the light source and the camera are along the same direction, be it $45\degree$ or $90\degree$, whereas the mirror is bright only when both the camera and the flash are at $90\degree$. In case (c), the images of the mirror and the retro-reflector are dark. On the contrary, the white paper is always slightly turned on despite the flash and camera positions because of the diffusion.  
%\todo{(a) When the LED is at $90\degree$, and the camera is at $90\degree$, both the retro-reflector and mirror areas are bright. (b) When the LED is at $45\degree$, and the camera is at $90\degree$, the retro-reflector and the mirror areas are dark, while the paper area is slightly bright due to diffused reflections. (c) When the LED (TX) is at $45\degree$ arrival of incidence, and the camera (RX) is at $45\degree$, the retro-reflector area (on the right) is bright, the mirror area (in the middle) is dark, and the paper area (on the left) is dark.} 
We notice that the brightness of the retro-reflector tends to be weaker than that of the mirror but more uniform. This is because the retro-reflector fabric is not perfect. \fyi{Further measurements show that such dispersion is severed when the incidence angle is over $\pm20\degree$, as shown in \figref{fig:rr-angle}.}

%\paragraph{Modulating Retro-reflector}
%Modulating retro-reflector (MRR)~\cite{mrr} consists of a retro-reflector and a modulator for optical communications. An MRR operates as a passive sources which transmits bits by varying the intensity of the reflected light beam. MRR is widely used in free space communication where the other side is a laser. Existing MRR systems~\cite{expensive,expensive2} is usually of a large size, and modulation is commonly achieved with a high-end electroabsorption modulator altering the absorption spectrum by applying an electric field. Consequently, such setting is ill-suited for our scenarios which require a low-cost solution.

The ability to bounce back light from any incidence angle leads to a favorable property of a retro-reflector: when the light source emits omni-directional lights, the retro-reflector will concentrate the lights as it reflects them. This is illustrated in \figref{fig:retro1}. From experiments, we empirically found that the concentrated energy is directly proportional to the size of the retro-reflector fabric, as shown in \figref{fig:retro2}. This property enables us to achieve higher reflected signal strength by using larger retro-reflector.
\begin{figure}[!th]
  \begin{center}
      \subfigure[Energy Concentration]{
        \includegraphics[width=0.46\columnwidth]{retro-reflector.pdf}\label{fig:retro1}
      } 
      \hfill
      \subfigure[Reflected Energy vs. Area]{
        \includegraphics[width=0.46\columnwidth]{retro_size.png}\label{fig:retro2}
	  }
%      \vspace{-1em}
      \caption{Energy concentrating property of a retro-reflector when the light source emits omni-directional lights and the relationship between reflected energy and the retro-reflector size. }\label{fig:retro}
  \end{center}
%  \vspace{-0.3in}
\end{figure}


\paragraph{Liquid Crystal Display (LCD)}
In terms of embedding information bits on the reflected light, special retro-reflector can alter the amplitude by electronically controlling the reflection or absorption using for example MEMS technologies \cite{expensive,expensive2}. In our case, we hope to use ordinary, off-the-shelf retro-reflector fabrics. In order to modulate the lights reflected by such fabric, we resort to a liquid crystal display that can pass or block light under the control of electrical field. 


\begin{figure}[th]
  \begin{center}
      \subfigure[LCD Principle \cite{eavesdrop2}]{
        \includegraphics[width=0.48\columnwidth]{lcdworks-crop.png}\label{fig:lcdworks}
      } 
      \hfill
      \subfigure[LCD Driver]{
        \includegraphics[width=0.46\columnwidth]{../illustrations/conventional_LCD_driver.eps}\label{fig:lcd-circuits}
	  }
%      \vspace{-1em}
      \caption{The structure and principle of LCD, and its typical driving circuits. }\label{fig:lcd}
  \end{center}
%  \vspace{-0.3in}
\end{figure}

An LCD is a multi-layer sandwich structure. At the two far ends of the LCD panel are two polarizer films. The two polarizers can be parallel or perpendicular to each other. In the middle are two glass electrodes that encompassing a layer of the nematic phase liquid crystals, as shown in \figref{fig:lcdworks}. 
An LCD works as follows: when the incoming light passes through the first polarizer, it becomes polarized. Depending on the actual liquid crystal state, the polarity of the light will be changed or remain unchanged. 
In the natural state of the liquid crystal, its molecules are twisted. It will change the polarity of the light passing through it. If an electric field is imposed (by the two surrounding glass electrodes) on the liquid crystal, its molecules will become untwisted. The polarity of the light will not be affected when passing through. The light will finally be passed or blocked by the second polarizer on the other end, depending the conformance of their polarity \cite{eavesdrop2}. %http://qxwujoey.tripod.com/lcd.htm} 
%The reason we see the coloured images are due to the colour filter, light passes through the filtered cells creates the colors. There is also a colour filter containing the 3 primary colours (red, green and blue). 
At a high level, the polarization changes as the voltage added on it. At a low voltage, the incoming light traverses the LCD to hit the retro-reflector, and reflected light also traverses the LCD; At a high voltage, the incoming light is rejected by the LCD. 


%\p{Charging and discharging circuitry, as we will use them in the energy reuse. }
%The LCD usually consumes a little amount of current, but requires a relatively high voltage. For example, the LCD we used would start to take effect at 2.0V, and the desired working voltage is as high as 10V. In practice, we found a voltage of 6.0V will work. \todo{Explain the circuits, especially the charging/discharging paths.} We notice that the LCD itself is capacitor. \todo{need to further explain it's consequence. Postpone to the energy reuse section.}


%However, one disadvantage of LCDs are their low refresh rate, e.g., 60 or 75 Hz, which is too low for data communication. Fortunately, we find \textit{LCD shutters} with much higher refresh rate (up to 1KHz \hl{cite}). Fig.~\ref{fig:retrolcd} shows the basic principle of a retro-reflector with an LCD coverage.


==> design__Jacky_Shen_s_conflicted_copy_2014-12-06_.tex <==
\section{\retro System Design}\label{design}
In this section, we describe our design of \retro in more detail. The system consists of a \reader and a \vitag, each of which contains the transmitting and receiving logic. We elaborate their design one by one, starting with the transmitter of the \reader. Its detailed diagram is shown in \figref{fig:diagram_reader}.

%The system consists of \readertx, \readerrx, \tagtx, and \tagrx. The first two belong to the \reader\ and the last two belong to the \vitag.  
\subsection{\readertx Design}
The \readertx employs a standard VLC design as in other work:  it performs encoding using an MCU and toggles the LED light to control the power amplifier. Specifically, we employ a 1MHz carrier and perform on-off keying (OOK) and Manchester coding. The communication bandwidth we use is 10kHz. 

Note that we may use even higher carrier frequency and larger communication bandwidth. We made the choice due to the limitation of ordinary commercial off-the-shelf LED we have. If we toggle at a faster rate, the amplitude difference between On and Off state will be too small to serve as an effective carrier. We use 10kHz bandwidth as it suffices applications we have in mind, e.g., send back the tag ID and certain sensor information it may carry.

%We next focus on the design of the other three components, elaborating on the key design choices. 


\begin{figure}[!th]
\centering
\includegraphics[width=\columnwidth]{fig/read_diagram.pdf}
\vspace{-1em}
\caption{Circuit diagram of \reader. }
\label{fig:diagram_reader}
\end{figure}

\subsection{\readerrx Design}\label{ssec:readerrx}
%\subsection{\reader Transmitter (\readertx)} \label{subsec:LEDtrans}

%As shown in Fig.~\ref{fig:sysdiagram} (b), the transmitter on \reader\ is composed of a crystal oscillator that runs at 1MHz\footnote{The fastest flickering rate of our LED is 1MHz},\remind{Later on when we say using only RC oscillator for energy savings, do we have any measurement of the energy consumption of a crystal oscillator? We need to provide the number. \hl{also the size requirement}} and an MCU followed by two amplifiers. The MCU-generated bits toggle the crystal oscillator to OOK the signal with Manchester encoding. The modulated signal will then be amplified and fed to a LED. To make sure the brightness of the LED does not pose a difference between the transmitting and not transmitting state, we add a DC component to the signal. The magnitude of the DC component is adaptable so that we can dim the brightness of the LED emission. In addition to the dimming support, flickers are avoided in \reader\ transmitter. We use 10kHz as the symbol rate, which far exceeds the frequency (200 Hz) below which human eyes will feel of fluctuations, which could disturbing and unacceptable. 

% We illustrate a typical packet the LED transmits in Fig.~\ref{fig:commdiagram}.

% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/layout2.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf An LED-transmitted Packet} \hl{blah}.}
% \label{fig:commdiagram}
% \vskip -0.05in
% \end{figure}

%\subsubsection{Challenges of \readerrx Design}
%\paragraph{Challenges of \readerrx Design}
The major challenges that arise in the design of the \readerrx are the following. First of all, the signal from the \vitag reflection is extremely weak, especially due to the use of the small retro-reflector on the \vitag. Second, the signal is severely interfered by other light and electrical sources. In particular, as the light sensor sits next to the LED, it is likely that there is leakage from downlink signals and carrier, in additional to the diffusing reflections from the ambient sources. Because of the close distance, the interference is several orders of magnitude greater than the actual reflected signal from the \vitag. As measured \fyi{in one implementation of 12W LED lamp}, the power of the \vitag-reflected signal is about $-80dBm$ \fyi{at 1.5 meters} while the \readertx emitted light signal can be up to $30dBm$. In fact, these interference could cause the \readerrx amplifiers to saturate without careful design. In practice, the light reflected by the movement of humans and other objects around also causes such interference. 
Thirdly, the converted electrical signal is also interfered by commercial FM radios that operate around 1MHz. The harmonics of the $50-60$Hz AC supply of the lighting infrastructure also matters, which is on par with the toggling rate (0.5kHz) of our LCD modulator. %The harmonics be relatively strong than the reflected signal.
%\remind{We may move this AC harmonics to the part explaining the performance differences between indoor and outdoor, as we do not have special treatment of this noise source. or do we???}
Last but not the least, our choice of using a small and low frequency RC oscillator at the \vitag, instead of high-precision oscillator (for sake of energy consumption reduction), makes the reflected signal suffer from clock offsets and drifts.   


In our design, we first try to isolate the receiving path, both the circuit and light sensor, from the transmitting path. In practice, we use 4-layer PCB and always ensure the wires are covered by two copper layers connected to ground. We also shield the light sensor to avoid leakage of the downlink signals. 

In the rest of this section, we elaborate the modular and algorithmic designs of \readerrx that overcome these challenges.  


%\subsubsection{Amplification and Demodulation}
%Since the received signal is extremely weak (the order of uV), we apply four successive RF amplifiers (gain>80dB), an active detector with a high-speed operational amplifier (gain=0dB) and a baseband amplifier (gain=100dB) to achieve superior total performance (gain>100dB). The detailed design is the following. 
\paragraph{Amplification and Demodulation}
As shown in \figref{fig:diagram_reader}, an external light sensor with a parallel inductor captures the \vitag signal and performs preliminary band-pass filtering. The photocurrent is then amplified by a subsequent preamplifier and further transmitted to the internal (\ie on the \reader board hosted within the lamp) amplifier and processing circuit. An impedance matching module is incorporated. 

The pair of transmission lines is relatively long, decoupling the front end and the subsequent processing unit.%and easily interferes with \textit{common-mode noises} such as the radio and AC harmonics. 
As the two wires are equally affected by the common-mode noises, we thus design a tuned differential amplifier as the first-stage internal amplifier. By subtracting the signals from the two wire, the differential amplifier effectively eliminates the common-mode noises. It further suppresses other off-band noises through LC resonance at 1MHz carrier frequency. As the reflected signal from \vitag\ is extremely weak, we further amplify it through two additional LC-structured amplifiers. The overall amplification gain is $80dB$. 
This signal then goes through a high precision envelope detector to pick up the baseband signal from the carrier. 
%, which realizes regular passive diode demodulation that picks out the baseband signal from the $1MHz$ carrier but with much lower distortions. 
Finally, the baseband signal is amplified and fed to the MCU, which performs analog-to-digital conversion and decoding therein. 

Note that the gain of the differential amplifier is programmable and controlled by the micro-controller. We also use two-stage amplifiers (instead of one-stage amplifier with very large gain) both with feedback mechanisms. These mechanisms helps pull the circuit state away from self-excitation. 


%\begin{figure*}[!t]
%\vskip -0.1in
%\centering
%{\footnotesize
%\begin{tabular}{ccccc}
%\epsfig{file=../illustrations/waveform1.eps, width=0.2\columnwidth} & \epsfig{file=../illustrations/waveform2.eps, width=0.2\columnwidth} & \epsfig{file=../illustrations/waveform3.eps, width=0.2\columnwidth} & \epsfig{file=../illustrations/waveform4.eps, width=0.2\columnwidth} & \epsfig{file=../illustrations/waveform5.eps, width=0.2\columnwidth}\\
%{(a) Normal} & {(b) Up-truncated} & {(c) Down-truncated} & {(d) Up and Down-truncated} & {(e) Average-drifted}\\
%\end{tabular}
%}
% \vskip -0.1in
%\vspace{1em}
%\caption{\footnotesize{\bf Varying Wave patterns.} Blah Blah.}
%\label{fig:dynamicRange}
%\vspace{-1em}
%\end{figure*}
%

%\begin{figure*}[!t]
%\centering
%{\small
%\begin{tabular}{cccc}
%\epsfig{file=../illustrations/waveform1.eps, width=0.22\columnwidth} & 
%\epsfig{file=../illustrations/waveform2.eps, width=0.22\columnwidth} & 
%\epsfig{file=../illustrations/waveform3.eps, width=0.22\columnwidth} & 
%\epsfig{file=../illustrations/waveform5.eps, width=0.22\columnwidth}\\
%{(a) Normal} & {(b) Top-truncated} & {(c) Bottom-truncated} & {(d) Average-drifted}\\
%\end{tabular}
%}
% \vskip -0.1in
%\vspace{1em}
%\caption{Possible Waveform patterns after baseband amplifier of \readerrx. \todo{Verify!! Is it from after baseband amp?}}
%\label{fig:dynamicRange}
%\vspace{-1em}
%\end{figure*}


\begin{figure}[!th]
  \begin{center}
      \subfigure[Normal]{
        \includegraphics[width=0.45\columnwidth]{../illustrations/waveform1.eps}\label{fig:waveform1}
      } 
      \hfill
      \subfigure[Top-truncated]{
        \includegraphics[width=0.45\columnwidth]{../illustrations/waveform2.eps}\label{fig:waveform2}
      } \\ \vspace{-1em}
      \subfigure[Bottom-truncated]{
        \includegraphics[width=0.45\columnwidth]{../illustrations/waveform3.eps}\label{fig:waveform3}
      } 
      \hfill
	  \subfigure[Average-drifted]{
        \includegraphics[width=0.45\columnwidth]{../illustrations/waveform5.eps}\label{fig:waveform5}
      } 
\vspace{-1em}
      \caption{Possible waveform patterns after the baseband amplifier of \readerrx. }\label{fig:dynamicRange}
  \end{center}
\vspace{-1em}
\end{figure}

%\subsubsection{Decoding and Handling Clock Drift}\label{subsubsec:clockoffset}
\paragraph{Decoding and Handling Clock Drift}
The clock offset and drift caused by the RC-clock of the \vitag bring challenges as we try to extract the timing information from the signal and perform the decoding at the same time. %First, we describe why common decoding methods do not work in our case.
There are several common decoding methods. One method is based on peak (or edge) detection. Its principle is to extract the extreme (discontinuous) points in the signal to detect clock beats. A second approach is averaging-based algorithm in which signal samples are averaged to generate a threshold, and samples above this threshold denote ones and below denote zeros. A third approach is symbol-based match filter that tries to match the waveform of one symbol and detects the convolution peaks to determine the accurate timing.

\begin{figure}[tb!]
\centering
\includegraphics[width=\columnwidth]{../figures/slidingWindow.eps}
\vskip -0.05in
\caption{All possible 3-bit patterns (left) and illustration of their actual voltage levels (middle), and corresponding matching templates (right) for edge detection. 
}
\label{fig:swmsmf}
\end{figure}


However, none of these methods work for us. 
Take for example the normal signal input waveform shown in \figref{fig:dynamicRange}(a). 
Due to the possible lag of the automatic gain control at the \readerrx, the high dynamic range of interference, we may obtain top- or bottom-truncated waveforms, as shown in \figref{fig:dynamicRange}(b) and (c), or both top- and bottom-truncated waveform (not shown due to space limit). Such situation would fail peak/edge detection algorithms. Similarly, the ambient brightness changes (e.g., caused by human body reflection) will likely cause a time-varying shift in average value, as shown in \figref{fig:dynamicRange}(d). This would fail the averaging-based approach. Furthermore, due to Manchester coding, one bit contains two chips -- a high volt chip followed by a low volt chip, or vice versa, indicating a `0' and `1', respectively. Other than an all `0' or all `1' sequence, the rising edge and the falling edge are not evenly spaced in time. %The correlation peak for such unevenly spaced chips will be skewed. 
%A typical example is three chips that contain one high-volt chip followed by two low-volt chips, in which case the correlation peak will be skewed, compared to the case where the voltage is high for one chip and low for the next. 
This results in two (and at most two) consecutive low (or high) voltage chips for bit sequence `01' (or `10'). 
A low voltage chip corresponds to the LCD discharging phase at the \vitag; Consecutive low chips thus correspond to continuous discharging of the LCD. As a result, the second low chip will have a lower voltage than the first one. Similarly, the second high chip will have a higher voltage than the first one in two consecutive high voltage chips. The consecutive low or high voltage chips and their corresponding voltage level are depicted in \figref{fig:swmsmf}. 
In the face of these distortions, the single-symbol match filter method will fail, because the correlation peak will be skewed for those unevenly spaced high/low voltage chips.

%\vskip 0.05in\noindent{\bf \hl{CDMA-based algorithms}} use a string of chips to represent one bit~\cite{abc1}, and does correlation on the receiver side to decode the bit by finding the peak of the correlation result. The algorithm can pinpoint the clock and hence decode the signal in a low SNR situation, but it is not suitable for low symbol-rate channels like the uplink in our case. 

%\vskip 0.05in\noindent{\bf One-symbol \qm{match filter} algorithms} try to match the wave form of the signal and detects the convolution peaks to determine the accurate timing. However, due to the rough equivalence of the LCD on the tag side that shapes a bit and a capacitor, the basic wave form tends to be sawtooth, as shown in Fig.~\ref{fig:dynamicRange} (a) when there is no top or bottom truncation. Further, as the bits are encoded in Manchester code, the rising edge and the falling edge are not necessarily symmetric in time. A typical example is three chips that contain one high-volt chip followed by two low-volt chips, in which case the correlation peak will be skewed, compared to the case where the voltage is high for one chip and low for the next. Therefore, the timing will be biased.


%\noindent\textbf{\textit{Sliding-window Multi-symbol Match Filter:  }}
We develop a novel algorithm, termed \textit{sliding-window multi-symbol match filter} algorithm, to decode the signals from Manchester coding that subject to a huge dynamic range. %The approach extends the one-symbol match filter to that with an addition regarding clock adjustment using a multi-symbol match filter. 
The basic idea is to avoid the biased timing caused by skewed correlation peaks in the conventional symbol-based match filter method, by matching \textit{all possible patterns} of the waveform that may result from Manchester encoding, and iteratively adjusting the local clock by every bit period. To begin with, the algorithm exploits standard correlation to detect the preamble of a packet. In our design, preambles last for a time period equivalent to 3 Manchester chips.
%\fyi{Preambles are a string of eight `1's in our design. Its chips are evenly distributed and alternating between high and low voltages, and hence can be accurately detected}
%, using the fact that the preamble is different from any possible bit patterns in the payload and is known beforehand. 
Upon finding the preamble, the algorithm estimates the length of a bit using the knowledge of the \vitag clock which is known but subject to offsets and drifting. Then the algorithm iteratively performs the following two steps:
\\[4pt]
\noindent\textit{Step 1: Template Matching.} For all the samples within the three-bit span, we match them against the corresponding template, as shown in \figref{fig:swmsmf}. Note that the template is of amplitude of $\pm1$, so as to most precisely detect the rising or falling edges of the bit in the middle. Ideally, the right correlation yields a peak in the middle of the three bits. 
\\[4pt]
\noindent\textit{Step 2: Local Time Recovery.} 
%Then the algorithm adjusts the clock estimation by correlating the three bits from the raw signal against the corresponding gold pattern from the eight patterns. 
Due to the time variance with the start of the packet and the frequency deviation between the clocks of the \reader and the \vitag, the peak correlation does not necessarily align with the actual timing of the edge. This yields errors in clock estimation. To bound this error as the decoding goes, we perform linear regression $t=k\cdot s+s_0$ to estimate the central time of every three bits, where $s_0$ is the initial time estimate after preamble detection, $s$ and $t$ are the central time from the \reader's view and from the \vitag's view, respectively, and $k$ denotes the clock sampling ratio of the \vitag\ over \reader. Every round $k$ is re-estimated, and then the algorithm moves the three-bit window one bit forward.
 
The whole procedure is repeated till reaching the end of the packet. This time recovery algorithm bounds the error on $t$ from diverging as the decoding process proceeds. %\todo{The proof does bounds $k$. Original text say prevent $k$ from propagating, which is not correct. How about simply put "This time recovery algorithm bounds the estimation error as the decoding proceeds."? Chao: yes, this is more appropriate} 
We formally describe this in the following lemma, for which we give a proof in Appendix.
\begin{lemma}
The time recovery algorithm ensures the error of the \vitag clock estimation to converge to zero asymptotically if a packet contains infinite number of bits. 
\label{lem:lemma1}
\end{lemma}

%Note that we choose a three-bit time span as a correlation unit because three bits are the smallest number of bits that contain all possible wave forms when the signal is Manchester-encoded. The use of three-bit window can maximize the correct detection of the bit in the middle. 


% \begin{figure}[!t]
% \vskip -0.03in
%   \centering
%       {
%         \epsfig{file=../figures/divide.eps, width=0.6\columnwidth}
%       }
% \caption{{\bf Signal Captured by the LED Light Sensor \hl{replace with a system block diagram!!}} \hl{integrates both mmm in a single design. It can operate using both RFID and TV transmissions}.}
% \label{fig:capture}
% \vskip -0.05in
% \end{figure}




%\begin{figure}[!th]
%  \begin{center}
%      \subfigure[Waveform of TP1]{
%        \includegraphics[width=0.4\columnwidth]{../illustrations/waveform_a1.eps}\label{fig:waveformOfTag_Lightsensor}
%      } 
%      \hfill
%%      \subfigure[Waveform of TP2]{
%%        \includegraphics[width=0.45\columnwidth]{../illustrations/waveform_a2.eps}\label{fig:waveformOfTag_Amp}
%%      } \\
%      \subfigure[Waveform of TP3]{
%        \includegraphics[width=0.4\columnwidth]{../illustrations/waveform_a3.eps}\label{fig:waveformOfTag_TunedAmp}
%      } 
%      \\
%	  \subfigure[Waveform of TP4]{
%        \includegraphics[width=0.4\columnwidth]{../illustrations/waveform_a4.eps}\label{fig:waveformOfTag_Dmodulator}
%      } 
%      \hfill    
%	  \subfigure[Waveform of TP5]{
%        \includegraphics[width=0.4\columnwidth]{../illustrations/waveform_a5.png}\label{fig:waveformOfTag_Thresholding}
%      } 
%
%%      \vspace{-1em}
%      \caption{Waveforms at various stages in the \tagrx. \todo{Pay attention to the units/scale. e.g., seems there is no much amplification from (a) to (b).}}\label{fig:waveformOfTag}
%  \end{center}
%%  \vspace{-0.3in}
%\end{figure}
%

\begin{figure}[!th]
\centering
\includegraphics[width=\columnwidth]{fig/tag_diagram.pdf}
\vspace{-1em}
\caption{Circuit diagram of \vitag.}
\label{fig:diagram_tag}
\end{figure}


\subsection{\tagrx Design}

%The major challenge we want to address in the \vitag design is to push to limit the low power consumption. For a normal design, there would be two major energy consumption modules, namely the ADC and digital signal processing (for the \tagrx) and the light emission and modulation (for the \tagtx). The adoption of the retro-reflector removes the energy for emitting light, the modulation (via LCD) still consumes relatively significant energy. In addition, a high accuracy crystal oscillator would incur significant energy overhead. 
For a normal design of \tagrx, the major energy consumption would be from the ADC and digital signal processing. 
In our design, we perform most of the processing in analog domain and avoid using the ADC while retaining accuracy. 

%As shown in \figref{fig:sysdiagram}, the incoming light signal is first captured by the light sensor (photodiode) and converted to electrical signal. The signal is first filtered and then go through tuned amplifiers and a demodulator. It is further amplified and then digitized via a comparator (instead of an ADC).  


%\subsubsection{Demodulation}
\paragraph{Demodulation}
As shown in \figref{fig:diagram_tag}, the incoming light is first captured by the light sensor. 
%As shown in Fig.~\ref{fig:sysdiagram} (b), we use two triode amplifiers combined with a well-designed detector to achieve high gain and extremely low power consumption. \vitag\ captures signals with a light sensor. 
The light sensor has an equivalent capacitance, which, with an inductor parallel to it, makes up a preliminary LC filter. Two triode amplifiers successively amplify the RF signal, after which the signal is passed along for demodulation. 

Our demodulator contains a constant voltage source and a low-pass amplifier. The constant voltage source sets a ultra-low quiescent current that flows into the base of the triode in the low-pass amplifier, making it work at a critical conduction mode, so that the positive half of the signal can pass through and be amplified while the negative part can only make the triode into cut-off mode. Hence, the 1MHz AC carrier is turned into the unipolar signal with a low frequency DC bias which can represent its primary envelope. Finally, the envelope signal is obtained by a smoothing capacitor and then fed into a comparator for digitization. 

%Overall, compared with a commonly used passive diode detector, much higher gain can be provided by our solution which simultaneously consumes quite low energy due to its critical conduction mode.

%\subsubsection{Digitization and Decoding}
\paragraph{Digitization and Decoding}
%While the output of the envelope detector is a smooth wave, it is still analog with continuous values. In principle, a receiver with an ADC can distinguish between the two signal levels by processing the digital samples. Specifically, say we have two signals with different voltages, $V_0$ and $V_1$, $V_0 > V_1$, where $V_0$ and $V_1$ correspond to the power levels for the zero and one bits. To distinguish between them, the receiver would first compute a threshold value. If the duty cycle of the signal is $50\%$, and odds of the occurrence of zeros and ones are equal, then the threshold is the average of the two power levels. If the received signal is greater than this threshold, we conclude that the received signal is $V_1$; else, we conclude that the received signal is $V_0$.
%\fye{To avoid using power-hungry ADCs, we digitize the analog signal with a comparator. Because of the pulse-width modulation (PWM) we adopted, the goal of our design is different from a typical digitization process that involves comparison instant value against the time-average. The PWM-encoded signal uses the width of a pulse to denote bits. Specifically, a wide pulse denotes 1, and a narrow one denotes 0. To align with this pattern, we design the comparator to detect the \textit{change} of the voltage. First, using a resister and a capacitor, the comparator sets a time constant that features its detection delay that corresponds to the input symbol rate. The comparator consistently compares the current (analog) signal voltage $V_{now}$ with that of the last symbol $V_{previous}$. If $V_{now} > V_{previous}$, the comparator outputs `1'; otherwise, it outputs `0'. }%It is easy to see that our design traces the relative changes in the voltage.}
\fyi{To achieve better energy efficiency, power-hungry ADCs should be avoid and MCU should not always be waking-up. We digitize the analog signal with a comparator. For most of the time, the CPU of MCU is sleeping with only one timer running to measure the time. When a positive jump appears on the TP4 shown in \figref{fig:diagram_tag} (i.e., output of the comparator), the CPU of MCU is waken up, and record the time stamp of the timer, then the CPU halt again. Together with the last wake-up time stamp, we can know the period of the clock cycle on the output of comparator. To align with this working pattern, we adopt clock-period coding. For example, a 185us clock period denotes 00, 195us clock cycle denotes 01, 205 us denotes 10, and 215us denotes 11. So we can receive 2 bits with MCU being waken up just one time.}
\fyi{This enables MCU to sleep most of the time, and upon waking up, it records the time stamp, determines the received bits, and goes into sleep mode again. In our implementation, with a MSP430 MCU running at 1MHz, these routines are done within $16us$. So when there is no carrier or no data on the carrier, the MCU sleep for all the time. When the Tag is receiving data, it still sleeps for most of the time, and just work 16us in the receiving cycle of 200us. }
%\todo{I'm not quite sure here. The comparator already outputs 0 or 1, why MCU needs to do it again? Can we annotate $V_{now}$ and $V_{previous}$ in the figure? If you're sure, keep it. } 
%Further, using a traditional passive diode detector would lead to jagged waveform, which would further cause false comparison results at any edge-based comparator. Instead, our comparator design is more suitable for Manchester coding, which is widely adopted for preventing long consecutive $1$s or $0$s in a bit stream, in avoidance of picking a threshold value that would suffer from drifting. 
%\fyi{When a new symbol comes in, MCU is waken up by the comparator output, and then judges the symbol by the continuously working internal timer.}

%\todo{Need serious double check. It seems to me the microcontroller actually performs decoding. If wrong, the highlighted text below needs to be changed accordingly. } %In the receiving phase, microcontroller consumes $120\mu A$.
%Therefore, we are able to use MSP430 working at its lowest frequency as the MCU. 

In summary, we achieve low energy reception at \vitag by using only analog elements and a low-power MCU (MSP430). The MCU is in sleep mode for most of the time. In the analog circuit design, we further set the transistors to work at a lower DC operating point to maximally reduce energy consumption. 




\subsection{\tagtx Design}\label{subsec:tagtrans}

%\begin{tcolorbox}
%\vskip 0.05in\noindent{\bf Challenge:} Transmitting with the LCD at a high toggling frequency consumes even more power than the receiver.
%\vskip 0.05in\noindent{\bf Solution Principle:} Recycle energy spared by the LCD at every toggle; And use an MCU internal RC oscillator instead of the crystal oscillator used in the receiving phase.
%\end{tcolorbox}


Our \vitag\ transmitter transmits by passively backscattering the incoming light. The core of the transmitter is the combination of an LCD and a retro-reflector that serves as a modulator. %To conserve energy, we design an energy reuse module that, in every modulation cycle, recollects $50\%$ of the energy that would have been wasted by the LCD without such a module. 
%To further save energy, instead of using power-demanding crystal oscillators, we use an MCU internal RC oscillator to generate control signals to toggle the LCD. While the RC oscillator does have worse clock stability and a lower frequency, we design modules that address these issues in~\ref{ssec:readerrx}. 
While the LCD has an ultra low quiescent current, more than $70\%$ of the power consumption during transmission is caused by LCD. The reason is that the LCD has a considerable equivalent capacitance ($~9nF$), which must be charged to $5.5V$ to turn the LCD off and be discharged to turn the LCD on. It is this charging-discharging process that consumes energy. To conserve energy, we design an energy reuse module that recycles the discharging current. 
The LCD requires a voltage high enough (\eg at least $5.5V$) to drive it to achieve desired polarization level. This high voltage is nearly 3 times of solar cell's voltage and cannot be directly fed by solar cells. We design a voltage boosting module that achieves this. The overall design of the \vitag transmitter is presented in \figref{fig:diagram_tag}. 

%We now break down the design into the following key points.

%\subsubsection{Modulating the Retro-Reflector with an LCD}
%To avoid actively generating light signals, which may cost way more power than affordable on a battery-free \vitag, we instead take the advantage of retro-reflectors that passively bounce the incoming light back. As described in Section~\ref{sec:background}, the retro-reflector has the merit that it can directionally bounce the light at a direction same as the one the light arrives at. To modulate the light, we cover the retro-reflector with an LCD. As electromagnetic waves hit the LCD, the LCD lets the light pass through or blocks it depending on the polarization, i.e., the orientation of the liquid-crystal molecules, in the LCD, which is controlled by the voltage added on it. If the applied voltage is large enough, the pixels will appear black. 
%The highest voltage applied to our LCD that turns it completely black is $6.1V$, and the lowest voltage with which it starts to be polarized is $2.1V$. We are able to flicker it as fast as $0.5kHz$, making a $200\mu A$ current consumption. Note, that there are other voltage-controlled reflective materials existing that may have higher flicking rate or lower power. Applying one of those in the system might enhance the energy efficiency and the capacity of the system.  

%\subsubsection{Energy Reuse}
\paragraph{Energy Reuse}
%While LCD has a ultra low quiescent current, more than 70\% power consumption of the circuit during the transmitting is caused by LCD. The reason is that LCD has a considerable equivalent capacitance(about 9nF in our case), which must be charged to 5.5V to turn LCD off and be discharged to reopen it. It is the charging-discharging process consumes those energy. Also the voltage, 5.5V, is nearly 3 times of solar cell's voltage, so a low quiescent and high efficiency DC/DC step-up circuit is needed. 
A conventional LCD driving circuit would discharge LCD from the high driving voltage to Ground and thus waste the energy. %If we can recollect this portion of the current during the LCD discharging phase, it will reduce significant power consumption of the whole circuit. In response, 
The design of our energy reuse module is depicted in Fig.~\ref{fig:energyreuse}.  
\begin{figure}[tg]
  \centering
      {
        \epsfig{file=../illustrations/EnergyReuseCircuits_2.eps, width=\columnwidth}
      }
\vspace{-1ex}      
\caption{Energy reuse design for LCD driver. }
\label{fig:energyreuse}
\end{figure}

During the charging phase, the DC/DC boosts voltage supplied by the solar cell to the high voltage needed for driving the LCD towards a blocking state. 
The MCU sets this high voltage on and activates the transistor $Q_0$ (the PNP transistor in the conventional LCD driver module).
%, and at the same time, the MCU sets a low voltage and ensures the NPN transistor $Q_1$ (on the discharging) to a cut-off state. 
This operation puts the LCD into the charging mode and will pump up the voltage of the LCD.
%This voltage, which the MCU sets to open through transistor $Q_0$ (assume $Q_0$ is the name of the PNP transistor in the conventional LCD driver block), applies to the LCD. Because $Q_1$ is set to close, the voltage on the LCD gets to pump up until it reaches the discharging phase.

In the discharging phase, the MCU sets the $Q_0$ to the cut-off state and thus closes the charging path, and activates the NPN transistor $Q_1$ on the discharging path. %Since there is a diode \fyi{(within $Q_1$???)} that \fyi{blocks the only path along which the LCD is supposed to discharge to the ground, the current that flows from the discharging LCD does not go straight to the ground.} 
Unlike a conventional LCD driver that discharges directly to the ground, in our design, the current flows back to the input of DC/DC circuits. This helps reduce the current drawn from the solar cell. Measurements show that the total power consumed by LCD while switching at $0.5kHz$ decreases from $84uA$ to $46uA$ with energy reuse. 

We note two things about our design. First, the two signals controlling the on/off state of LCD are generated by an MCU, and is alternately activated with a short interval ($2us$). This ensures only one transistor of $Q_0$ and $Q_1$ is open at a time and avoids the transient high current that would be caused if both semi-conductive transistors are activated during the switching. Second, the diode $D_0$ is critical. It prevents the charge on the LCD from discharging to the solar cell. Without it, the initial high voltage ($5.5V$) of LCD will be pull down to that of the solar cell ($2.1V$) immediately after $Q_1$ is ON, a high transient current would result and most energy would be wasted on the BE junction of $Q_1$.
%there will be a transient high current that pull the voltage on LCD to the voltage of solar cell immediately after , thus waste most energy on the b-e junction of transistor $Q_1$. 



==> intro_0.tex <==
\section{Introduction}

\begin{figure}[!t]
\vskip -0.03in
  \centering
      {
        \epsfig{file=../figures/prototype-photo.eps, width=0.6\columnwidth}
      }
\caption{{\bf Our \vitag\ Prototype} \hl{integrates both mmm in a single design. It can operate using both RFID and TV transmissions}.}
\label{fig:tag}
\vskip -0.05in
\end{figure}

LEDs are prevalently deployed for illumination. This ubiquity opens a door for the LEDs to communicate with small computing devices through the vehicle of visible lights. The last few years have seen significant advances in VLC systems --- VLC systems today can achieve bit rates up to \hl{ss Mbps} from an LED transmitter to a receiver over a distance of \hl{ss}~\cite{flawedsys1,flawedsys2,flawedsys3,flawedsys4}. Researchers have also demonstrated the capability of providing location services using VLC~\cite{location1,location2}. These impressive capabilities are made possible by systems that encode and modulate the light emitted by the LED. However, all these systems, on one hand, either support only one-directional communication from the LED to the device where the device does not have the transmission capability, or entail the mobile device having additional LED~\cite{led2led1} or Bluetooth~\cite{ble1} facilities to transmit the uplink data; On the other hand, achieving such high data rate requires complicated modulation schemes and power-expensive analog-to-digital converters (ADCs) that consume power on the order of \hl{10mW}~\cite{flawedsys1}; this is orders of magnitude more power than is available on handhold devices that harvest power from ambient light sources.

In this paper, we ask if it is possible to achieve a bi-directional communication system on battery-free mobile devices only using the visible light as the carrier. Such a system would not only work at any location with LEDs at any time, but would also remedy the security flaws typically faced by existing RFID systems, where the uplink transmission tends to be exposed to a wide area of space, leaving chances for sniffers and attackers to temper the system. Thus, a positive answer would enable ubiquitous communication with access to existing network infrastructures at unprecedented spacial and temporal scales with user security preservation. 

Designing such a system, however, is challenging as (1) generating light waves and modulating them typically require much more power than can be harvested from ambient light sources by a small device (see~\ref{sec:app}), and moreover, (2) detecting signals sent by the device at the LED receiver against interferences is hard. In this paper, we introduce \vitag, a VLC system that provides duplex communication capabilities on battery-free devices only using visible light carriers. To address the challenge of detecting signals against interferences on the LED receiver, \vitag\ uses a novel algorithm specifically designed for the LCD-modulated signals. Instead of generating signals, \vitag\ addresses the power constraint challenge by backscattering the incoming light waves using retro-reflectors and modulating using Liquid-Crystal Displays (LCDs). This helps the backscattered signal focus at the receiver on the LED, and avoids generating signals on \vitag. In addition, \vitag\ recycles the LCD modulation energy with an energy reuse module, further optimizing the mobile device size to the size of a regular credit card. Finally, there are a set of other techniques behind the \vitag\ design that make it feasible in real-world illumination system deployment, which we will describe in later sections.

\textbf{\vitag.} To understand our \vitag\ design on battery-free ID card-sized tags, consider an LCD whose emitted light can be manipulated by an additional small circuit inside the light bulb. This circuit embeds information in the light and modulates it, while keeping the brightness of the light the same without any flickering. On the \vitag\ side, a light sensor captures the light signal that conveys information from the LED. To conserve energy, \vitag\ only uses analog components to demodulate the signal without an ADC. Upon detecting data, a low-power micro-controller on \vitag\ is waked up for uplink data transmission. It drives up the LCD to flicker, therefore sending data back to the LED by backscattering the light with a retro-reflector behind the LCD. This uplink data can be captured by a light sensor placed on the LED, along with interferences caused by downlink transmission, nearby human and object movements, household electricity fluctuations, and so on. A specifically designed receiver associated with the LED then performs the time recovery and demodulates the signal. To get a network of \vitag\/s and LEDs into play, we design a Media Access Control (MAC) protocol to mediate the communications in LEDs' illumination range. 

To show the feasibility of our ideas, we have built a hardware prototype, shown in Fig.~\ref{fig:tag}, that is approximately the size of a credit card. Our prototype includes multiple off-the-shelf LEDs emitting white lights, LED transmitters each stuffed inside an LED, LED receiver PCBs and \vitag\ PCBs. LEDs and \vitag\/s are equipped with a micro-controller, respectively. Our prototype also includes a solar cell of size \hl{ss $\times$ ss} on \vitag.

We evaluate our system in locations where illuminating LEDs are typically deployed, including office settings and evenings, as well as a dark chamber without other light sources as the baseline. We measure the longest communication range between the LED and \vitag, the area in which \vitag\ uplink transmission can be sniffed or tempered, and concurrent transmission capabilities. Our experiments show the following:

\begin{Itemize}
\item  Our \hl{ss $\times$ ss} \vitag\ prototype can achieve a bit rate of \hl{10kbps} on the downlink and \hl{1kbps} on the uplink at distances of up to \hl{2.2m} in dark chambers, \hl{2.0m} on sidewalks in the evening, and \hl{ss m} in offices, under the power budget of \hl{bb $\mu W$}.
\item \vitag's uplink transmission cannot be detected over the radius of \hl{m}, and malicious readers cannot detect uplink transmissions when tempering \hl{m} away from working \vitag\/s.
\item Via the MAC protocol described in Section~\ref{sec:mac}, \hl{blah}
\end{Itemize}

\vskip 0.05in\noindent{\bf Contributions:} We make the following contributions:
\begin{Itemize}
\item We present \vitag, the first visible light duplex communication system design that operates on battery-free devices while retaining a small size for them.
\item We develop a secure communication primitive applicable to RFID systems that acts against side sniffers and malicious transmitters.
\item Finally, we present designs and build a prototype which shows how all of the above, from \vitag, modified LEDs, through to the network stack, can be implemented on credit-card sized battery-free devices at a low cost.
\end{Itemize}




==> intro_2.tex <==
\section{Introduction}

\begin{figure}[!t]
\vskip -0.03in
  \centering
      {
        \epsfig{file=fig/sysdiagram-eps-converted-to.pdf, width=0.6\columnwidth}
      }
\caption{{\bf Our \vitag\ Prototype} \hl{integrates both mmm in a single design. It can operate using both RFID and TV transmissions}.}
\label{fig:tag}
\vskip -0.05in
\end{figure}

%\p{VLC is promising direction}
Nowadays, LEDs have been prevalently deployed for illumination purpose for its advantageous properties such as high energy efficiency, long lifetime, environment friendliness, to name a few. Being semiconductor devices, LEDs also possess another feature, i.e.\, it can be turned on and off instantaneously. This effectively turns LED lights into a carrier and gives rise to a new ''dual-paradigm'' -- illumination and communication -- of LED lighting. Thanks to the ubiquity of lighting infrastructure, visible light communication (VLC) has thus attracted lots of research interest~\cite{fundamental1, fundamental2, standard}. A standard (IEEE 802.15.7) has been established recently~\cite{standard} to ensure inter-operation among device manufacturers. Some practical systems such as ByteLight~\cite{ble0} have debuted the exploitation of LED lighting infrastructures for both communication and localization~\cite{location1,location2}. 

%\p{existing solution does not meet two-way communication need}
Existing work has primarily focused on exploring or improving the one-way link from the LEDs to the mobile ends, i.e.\, from the LEDs to the receiving small computing devices. Indeed, significant advances have been made, e.g.\, VLC systems today can achieve bit rates up to $~10Mbps$ from an LED transmitter to a receiver over a distance of $~10km$~\cite{expensive,expensive2,retro1,retro2}. However, despite these promising results, it solves only half of an actual communication system where two-way communications are essential. In response, in ByteLight and many other smart light system with remote control, a BlueTooth Low Energy link is typically leveraged as the uplink to send information or control messages from a mobile device to the light. 

%\p{The need of low-power solution, not affordable to use LED at mobile device.}
The dual-paradigm nature of LED lighting, with illumination as the primary goal, naturally leads to an asymmetric communication setting. The transmitters, i.e., LEDs, are externally powered and can emit strong signals, whereas the receivers are typically small computing devices such as mobile phones and even weaker sensors. Applying the LED-photodiode link straightforwardly from a mobile device or sensor node to the lighting LED is not affordable. A typical VLC system consists of an LED, a photodiode and intermediate optical components (e.g., lenses). To achieve high speeds as reported in literatures~\cite{expensive,expensive2,flawedsys3,flawedsys4}, special and expensive hardware pieces such as multiple quantum well electro-absorption modulators and lasers have to be used~\cite{expensive}; They consume orders of magnitude more power than is available on credit-card-sized devices that harvest energy from LED lights~\cite{solarsheet}. In this light, we focus on using ordinary lighting LEDs whose primary goal is illumination. In such a setting, the LED flickering rate is relatively low. For instance, we measured that the rising and falling frequency of an ordinary commodity LED bulb is at most $1MHz$.

% \fye{
% This ubiquity opens a door for the LEDs to communicate with small computing devices with the emitted lights. The last few years have seen significant advances in VLC systems --- VLC systems today can achieve bit rates up to \hl{ss Mbps} from an LED transmitter to a receiver over a distance of \hl{ss}~\cite{flawedsys1,flawedsys2,flawedsys3,flawedsys4}. Researchers have also demonstrated the VLC capability of providing location services~\cite{location1,location2}. These impressive capabilities are made possible by systems that encode and modulate the light emitted by the LED. However, all these systems, on one hand, either support one-directional communications only from the LED to the device, or require the mobile device to have additional LED~\cite{led2led1}, Bluetooth~\cite{ble1} or other facilities~\cite{retro1,retro2} to transmit the uplink data; On the other hand, achieving such high data rate requires complicated modulation schemes and power-expensive analog-to-digital converters (ADCs) that consume power on the order of \hl{10mW}~\cite{flawedsys1}, alongside the power needed for driving those facilities; this is orders of magnitude more power than is available on credit card-sized devices that harvest power from ambient light sources~\cite{solarsheet}.
% }

% \p{our goal -- very low power bi-directional VLC, low enough to be affordable by harvesting energy from the LED light. Compared with RFID, it has more favorable security features. }
In this paper, we ask if it is possible to achieve very low power bi-directional VLC where the mobile end is affordable solely by harvesting energy from the LED light. Such a system would not only work at any location with LEDs at any time, but would also remedy the security flaws typically faced by existing RFID systems, where the uplink transmission tends to be exposed to a wide area of space, leaving chances for sniffers and attackers to temper the system. Thus, a positive answer would enable ubiquitous communication with access to existing network infrastructures at unprecedented spacial and temporal scales with user security preservation. 

%\p{core idea: leverage the retro-reflector to avoid the need of generating high power visible light; use LCD to modulate the reflected lights. }
Our core idea is as follows. To avoid generating power-expensive visible lights on the mobile end, we use a toggling \textit{Liquid-Crystal Display (LCD)} to modulate a \textit{retro-reflector} that directionally bounces the incoming light back to the LED, which forms a low-power uplink.   

%\p{challenges in achieving the low-power goal: 1) energy consumption at the receiver side; 2) LCD energy consumption at high toggling frequency at the transmitter side; 3) weak signal detection; 4) clock-drift handling at the LED side, without explicit synchronization between transmitter and receiver. }
Designing such a system, however, is challenging for the following reasons:
\begin{Itemize}
\item Demodulating and decoding the high throughput LED-transmitted data is power consuming. 
\item Transmitting with the LCD at a high toggling frequency consumes even more power than the receiver.
\item The LED has to detect retro-reflected signals 3 orders of magnitude weaker than its interfering transmissions.
\item The LED must handle clock offsets on the mobile end that uses a low-cost clock with low oscillating frequency.   
\end{Itemize}
%as (1) generating light waves and modulating them typically require much more power than can be harvested from ambient light sources by a small device (see~\ref{sec:app}), and moreover, (2) detecting signals sent by the device at the LED receiver against interferences is hard. In this paper, we introduce \vitag, a VLC system that provides duplex communication capabilities on battery-free devices only using visible light carriers. To address the challenge of detecting signals against interferences on the LED receiver, \vitag\ uses a novel algorithm specifically designed for the LCD-modulated signals. Instead of generating signals, \vitag\ addresses the power constraint challenge by backscattering the incoming light waves using retro-reflectors and modulating using Liquid-Crystal Displays (LCDs). This helps the backscattered signal focus at the receiver on the LED, and avoids generating signals on \vitag. In addition, \vitag\ recycles the LCD modulation energy with an energy reuse module, further optimizing the mobile device size to the size of a regular credit card. Finally, there are a set of other techniques behind the \vitag\ design that make it feasible in real-world illumination system deployment, which we will describe in later sections.

%\p{our design: principles -- 1) use analog components as much as possible (to avoid ADC) and complicated digital signal processing; 2) circuit design to recycle energy for lcd; 3) differential amplifier design? 4) windowed multi-symbol match filter}
To address these challenges, we apply the following design principles:
% \begin{Itemize}
% \item Use differential tunning analog components and avoid complicated digital signal processing on the mobile end to conserve energy while achieving comparable accuracy to when ADCs are used. 
% \item Recycle energy spared by the LCD at every toggle.
% \item Design amplifiers that work at an almost cut-off state to further reduce energy consumption.
% \item Design a sliding-window multi-symbol match filter algorithm to remedy clock drifts and LCD-caused signal distortions.
% \end{Itemize}

\begin{Itemize}
\item Use analog components over digital ones while achieving comparable accuracy.
\item Recycle LCD energy. 
\item Design energy efficient amplifiers.
\item Design algorithms to decode signals that suffer from severe clock offsets caused by low-cost mobile end.
\end{Itemize}

%\textbf{\retro.} To understand our \vitag\ design on battery-free ID card-sized tags, consider an LCD whose emitted light can be manipulated by an additional small circuit inside the light bulb. This circuit embeds information in the light and modulates it, while keeping the brightness of the light the same without any flickering. On the \vitag\ side, a light sensor captures the light signal that conveys information from the LED. To conserve energy, \vitag\ only uses analog components to demodulate the signal without an ADC. Upon detecting data, a low-power micro-controller on \vitag\ is waked up for uplink data transmission. It drives up the LCD to flicker, therefore sending data back to the LED by backscattering the light with a retro-reflector behind the LCD. This uplink data can be captured by a light sensor placed on the LED, along with interferences caused by downlink transmission, nearby human and object movements, household electricity fluctuations, and so on. A specifically designed receiver associated with the LED then performs the time recovery and demodulates the signal. To get a network of \vitag\/s and LEDs into play, we design a Media Access Control (MAC) protocol to mediate the communications in LEDs' illumination range. 

%\p{We demonstrated the design with a batter-free ViTag by harvesting LED light energy. We explore the tradeoff between the solar panel area and retro-reflector area to achieve a maximum working range for a typical lux level. }\todo{This suggests that the optimal value be a function of the solar cell efficiency and the reflecting concentration ratio.}
We demonstrated the design with a battery-free credit-card-sized \textbf{\vitag}, as shown in Fig.~\ref{fig:tag}, that harvests energy of off-the-shelf LED lights. We also explored the tradeoff between the solar panel area and the retro-reflector area for achieving a maximum working range at a typical $lux$ level. 
%To show the feasibility of our ideas, we have built a hardware prototype, shown in Fig.~\ref{fig:tag}, that is approximately the size of a credit card. Our prototype includes multiple off-the-shelf LEDs emitting white lights, LED transmitters each stuffed inside an LED, LED receiver PCBs and \vitag\ PCBs. LEDs and \vitag\/s are equipped with a micro-controller, respectively. Our prototype also includes a solar cell of size \hl{ss $\times$ ss} on \vitag.

We evaluate our system in locations where illuminating LEDs are typically deployed, including offices and evening streets. We also evaluate in dark chambers as the baseline. We measure the maximum communication range between the LED and the \vitag\ in varying $lux$, \vitag\ orientation, angle of incidence, solar panel area and retro-reflector area settings. Our experiments show that our \hl{ss $\times$ ss} \vitag\ prototype can achieve a bit rate of \hl{10kbps} on the downlink and \hl{1kbps} on the uplink at distances of up to \hl{2.2m} in dark chambers, \hl{2.0m} on sidewalks in the evening, and \hl{1.5 m} in offices, under the power budget of \hl{400 $\mu W$}. We also evaluate the area in which \vitag\ uplink transmission can be sniffed or tempered. Experiments show \vitag's uplink transmission cannot be detected over the radius of \hl{m}, and malicious readers cannot detect uplink transmissions when \hl{m} away from \vitag\/s.

%\p{contributions: 1) propose the use of retro-reflector for practical two-way VLC; 2) address various challenges; 3) build and evaluate a real prototype system.}
\vskip 0.05in\noindent{\bf Contributions:} We make the following contributions:
\begin{Itemize}
\item We propose the first practical bi-directional VLC primitive that works for small battery-free devices using retro-reflectors and LCDs and ordinary white LEDs.
\item We address various challenges by designing energy-efficient components on the \vitag\ and an unsynchronized decoding scheme on the LED.
\item Finally, we build and evaluate a prototype system which shows all of the above.
\end{Itemize}
%\begin{Itemize}
%\item We present \vitag, the first visible light duplex communication system design that operates on battery-free devices while retaining a small size for them.
%\item We develop a secure communication primitive applicable to RFID systems that acts against side sniffers and malicious transmitters.
%\item Finally, we present designs and build a prototype which shows how all of the above, from \vitag, modified LEDs, through to the network stack, can be implemented on credit-card sized battery-free devices at a low cost.
%\end{Itemize}




==> intro_liqul.tex <==
\section{Introduction}

%\begin{figure}[!t]
%\vskip -0.03in
%  \centering
%      {
%        \epsfig{file=prototype-photo.eps, width=0.6\columnwidth}
%      }
%\caption{{\bf Our \vitag\ Prototype} \hl{integrates both mmm in a single design. It can operate using both RFID and TV transmissions}.}
%\label{fig:tag}
%\vskip -0.05in
%\end{figure}

%Due to the scarcity of radio spectrum, visible light communication (VLC) has attracted increasing research attention since the last decade due to the extra wide spectrum (i.e., from 400-800 THz) and the safety advantages of visible lights~\cite{expensive,expensive2,retro1,retro2,fundamental1, led2led1, standard}.  Significant results have been achieved, e.g.\, 3.8Gbps at 1m distance, 10Mbps at 10km using specialized devices and high power lights \cite{??,??}. A standard (IEEE 802.15.7) has been established recently~\cite{standard} to ensure inter-operation among devices from different manufacturers. 

%For illumination, white LEDs are commonly used. The instantaneous On/Off feature turns LEDs into effective transmitters for visible light communication (VLC). Specifically, information bits can be embedded on the light by modulating the on/off state of the LED with on-off keying (OOK) or variable pulse-position modulation (VPPM) \cite{standard}. To receive such signals, while in some cases a cell phone camera or a digital camera will be sufficient \hl{need citations, ipsn14 and mobicom14}, photodiodes are generally used, because phone cameras can only achieve around 0.25MHz sampling rate~\cite{camera1} (in other words, low data rate), whereas photodiodes have generally higher bandwidth up to 0.5GHz~\cite{pdsheet}. Moreover, compared with a phone camera, the SNR of the photodiode is orders of magnitude higher at the same distance \hl{ipsn14}. 

%A typical way to generate white lights is to use a phosphor material to convert monochromatic lights from blue or ultraviolet to broad-band white lights, where the color of the monochromatic light depends on the band gap energy of the materials forming the p-n junction in the LED. 


Nowadays, white LEDs have been prevalently deployed for illumination purpose for its advantageous properties such as high energy efficiency, long lifetime, environment friendliness, to name a few. Being semiconductor devices, LEDs also possess another feature, i.e.\, it can be turned on and off \textit{instantaneously}. This effectively turns LED lights into a carrier and gives rise to a new ''dual-paradigm'' -- illumination and communication. 
The ubiquity of lighting infrastructure makes this dual-paradigm VLC (i.e., communication over existing lighting infrastructure) especially well suited to communicate with mobile devices or sensor nodes, e.g., streaming video to one's mobile phone or to collecting environment data from home sensors. 

For any communication system or link, it is essential to have bi-directional communication capability to ensure reliability and flexibility. A minimum requirement would be able to acknowledge correct or incorrect receiving of packets. To realize bi-directional communication, a straightforward way is to put together two one-way communication links. Unlike existing radio communication systems where the radio front-end is shared for both transmitting and receiving, a VLC system uses an LED for transmitting and use a light sensor (e.g., photodiode) for receiving. In consequence, existing work on VLC has primarily focused on improving the throughput for one-way link using power hungry, expensive, and dedicated devices \cite{expensive,expensive2,retro1,retro2}.  

However, the dual-paradigm nature of the system, with illumination being the primary goal, naturally leads to an asymmetric communication setting. On the one end is the externally powered LED, on the other end is the power-constrained device such as mobile phones and even weaker sensor nodes. Such an asymmetric setting makes it \textit{unfit} to symmetrically put two one-way communication links because the weak end cannot afford the power-intensive LED. Even if an LED were used, the glaring light would be very annoying to human eyes. In fact, some early VLC-based practical systems such as ByteLight~\cite{ble0}, which exploits LED lighting infrastructure for both communication and localization~\cite{location1,location2}, have adopted another medium (e.g., Bluetooth Low Energy (BLE)) for the device-to-LED communication, i.e., \textit{uplink}. This unfortunately incurs additional cost, bandwidth and system complexity. Also, the adoption of BLEs or LEDs for the uplink implies nearly omni-directional emissions, which accounts for extra power demand on the uplink. 
% A typical VLC link thus further includes intermediate optical components (e.g., lenses) for concentrating light. This leads to highly directional VLC systems and makes the actual design of a dual-paradigm VLC system deviate from those dedicated VLC systems aiming at extreme high data rate. 

In this paper, we present the design and implementation of \textit{\retro -- a low-power duplex VLC system}. Inspired by recent work on backscatter communication systems~\cite{abc1,abc4}, we avoid the usage of an LED for the uplink communication by backscattering the incoming light from the lighting LED. Central to \retro\ is the adoption of retro-reflecting material which can bounce back light of an arbitrary incidence angle \textit{along its incoming path}. This essentially forms an uplink that concentrates energy without other concentrating optical elements. We further modulate the reflected light by applying an LCD as a modulator. By tuning the translucence of the LCD, we control the passing of the light reflected by the retro-reflector, and encode information bits using On-Off-Keying (OOK). The modulated reflected light is then picked up by the photodiode on the LED side and decoded by a dedicated system.


%Enabling asymmetric low-power VLC communication is non-trivial. While the downlink is with powerful LEDs that can emit strong signals, the main challenge lies in the uplink. Applying existing LED-photodiode link straightforwardly to a mobile device or sensor node is not affordable. A typical VLC link consists of an LED, a photodiode and intermediate optical components (e.g., lenses). Existing work shows that one-way VLC link today can achieve bit rates up to $~10Mbps$ from an LED transmitter to a receiver over a distance of $~10km$~\cite{expensive,expensive2,retro1,retro2}. To achieve such high speeds, special and expensive hardware pieces such as multiple quantum well electro-absorption modulators and lasers have to be used~\cite{expensive}. Moreover, they consume orders of magnitude more power than is available on a low-power device. Using low-power LEDs \cite{} at tags seems a viable solution which however unfits our applications, which is detailed in Section~\ref{sec:proto}. 

%In this work, we propose a novel approach by toggling an \textit{LCD} to modulate a \textit{retro-reflector} directionally bouncing back the incoming light from the LED, which forms a low-power uplink. Our prototype is shown in Fig.~\ref{fig:tag}. By tuning the translucence of the LCD, we control the light perceived by the phtodiode at the LED side, encoding digital information using On-Off-Keying (OOK). The current consumed by the tag with a LCD modulator as well as a microcontroller is slightly above $200\mu A$. In other words, the tag can even be powered by a badge-size solar panel harvesting energy solely from the LED light. Downlink transmission is accomplished also in OOK with a LED bulb and a photodiode on the tag. Despite its low power consumption, designing such a system, however, is challenging for the following reasons:

%\note{liqul: These bullets are too low-level for ordinary reviewers. Make them more concise as well.}

To achieve low power consumption, we identify and overcome several challenges as follows: 1) power consumption of LCD; To push to the extreme the low power consumption; 2) weak signal detection at LED; 3) clock offset handling

% \begin{Itemize}
% \item Handling the high throughput LED-transmitted data is power consuming. 
% \item Transmitting with the LCD at a high toggling frequency consumes even more power than the receiver.
% \item The LED receiver must handle clock offsets from the mobile end with low clock oscillating frequency.
% \item The LED receiver has to detect retro-reflected signals 3 orders of magnitude weaker than interfering LED transmissions.  
% \end{Itemize}

%\note{liqul: put using BLE for upper-link communication into discussion.}

To address these challenges, we apply the following design principles:

\begin{itemize}
\item Use analog components over digital ones while achieving comparable accuracy; Design low-power amplifiers.
\item Recycle LCD energy. 
\item Avoid using crystal oscillators when transmitting.
\item Design algorithms to decode signals that suffer from severe clock offsets.
\end{itemize}

%\textbf{\retro.} To understand our \vitag\ design on battery-free ID card-sized tags, consider an LCD whose emitted light can be manipulated by an additional small circuit inside the light bulb. This circuit embeds information in the light and modulates it, while keeping the brightness of the light the same without any flickering. On the \vitag\ side, a light sensor captures the light signal that conveys information from the LED. To conserve energy, \vitag\ only uses analog components to demodulate the signal without an ADC. Upon detecting data, a low-power micro-controller on \vitag\ is waked up for uplink data transmission. It drives up the LCD to flicker, therefore sending data back to the LED by backscattering the light with a retro-reflector behind the LCD. This uplink data can be captured by a light sensor placed on the LED, along with interferences caused by downlink transmission, nearby human and object movements, household electricity fluctuations, and so on. A specifically designed receiver associated with the LED then performs the time recovery and demodulates the signal. To get a network of \vitag\/s and LEDs into play, we design a Media Access Control (MAC) protocol to mediate the communications in LEDs' illumination range. 

To demonstrate the effectiveness of \retro\ design, we implement a battery-free tag device, which operates by harvesting the energy of incoming light. The tag device is the same size of a credit card, one-third of the area is the retroreflector and two-thirds is the polycrystalline silicon solar cell. %\todo{describe the performance of the tag, e.g., working range, bit rate, etc.}
\figref{fig:system} depicts the tag.
We also explored the tradeoff between the solar panel area and the retro-reflector area for achieving a maximum working range in the worst case where the LED is the only light source, \ie no ambient light. %\todo{This suggests that the optimal value be a function of the solar cell efficiency and the reflecting concentration ratio.} 
\begin{figure}[th]
   \centering
   \includegraphics[width=.9\columnwidth]{system.pdf}
   \caption{System architecture (can be put side by side with the hardware prototype).}
   \label{fig:system}
   \vskip -3mm
\end{figure}

%We demonstrated the design with a battery-free credit-card-sized \textbf{\vitag}, as shown in Fig.~\ref{fig:tag}, that harvests energy of off-the-shelf LED lights. We also explored the tradeoff between the solar panel area and the retro-reflector area for achieving a maximum working range at a typical $lux$ level. 

We evaluate our system in locations where illuminating LEDs are typically deployed such as office environments. We also evaluate in dark chambers as the baseline. We measure the maximum communication range between the LED and the \vitag\ with various LED illuminations, \vitag\ orientations, solar panel areas and retro-reflector areas. Our experiments show that our $8.2cm\times 5.2cm$ \vitag\ prototype can achieve $10kbps$ on the downlink and $1kbps$ on the uplink at distances of up to $2.2m$ in dark chambers and $1.5m$ in offices, under the power budget of 400$\mu W$. We also evaluate the area around the \vitag\ in which uplink transmissions can be sniffed. Experiments show \vitag's uplink transmission cannot be detected outside of a spindle-shaped area of a radius $0.2m$.

%\p{contributions: 1) propose the use of retro-reflector for practical two-way VLC; 2) address various challenges; 3) build and evaluate a real prototype system.}
\paragraph{Contributions} 
We make the following contributions:
\begin{itemize}
\item We propose the first practical bi-directional VLC primitive that works for small battery-free devices using retro-reflectors and LCDs and ordinary white LEDs.
\item We address various challenges by designing energy-efficient components on the \vitag\ and an unsynchronized decoding scheme on the LED.
\item Finally, we build and evaluate a prototype system which shows all of the above.
\end{itemize}
%\begin{Itemize}
%\item We present \vitag, the first visible light duplex communication system design that operates on battery-free devices while retaining a small size for them.
%\item We develop a secure communication primitive applicable to RFID systems that acts against side sniffers and malicious transmitters.
%\item Finally, we present designs and build a prototype which shows how all of the above, from \vitag, modified LEDs, through to the network stack, can be implemented on credit-card sized battery-free devices at a low cost.
%\end{Itemize}




==> network.tex <==
\section{Media Access Control}
\label{sec:mac}

The discussion so far focuses on the communication aspects of a single \vitag-\reader\ pair. However, when many of these devices are in range of each other, we need mechanisms to arbitrate the channel between them. Unlike traditional RFID, the communication uplink from \vitag\ to \reader\ is highly directional because of the retro-reflectors. In addition, as a system with multiple access points that connect to the Internet, which is also different from RFID systems, \vitag\ needs mechanisms to provide roaming support. In this section, we explore the Media Access Control (MAC) design for \vitag\ and \reader\ with a break-down into four scenarios, namely, one \reader\ to multiple \vitag\/s, multiple \vitag\/s to one \reader, multiple \reader\/s to one \vitag, and one \vitag to multiple \reader\/s.

\subsection{One \reader\ to Multiple \vitag\/s}
\label{subsec:onereaderto}
One of the problems is how a \reader\ identifies a \vitag\ with a specific serial number from a number of \vitag\/s in range. This is necessary because if multiple \vitag\/s respond simultaneously to a query from \reader, they will jam each other. In \vitag, we set all \vitag\/s in a passive state, waiting for polling requests sent by \reader. When the serial number of a tag is called, the tag with this serial number responds within an assigned time slot. The rest of the \vitag\/s will ignore the payload that follows the serial number in the query as they notice that the serial number do not align with their own. For the requested \vitag\ to respond, it only needs to modulate the LCD and \textit{directionally} sends information back to the \reader\ that initiated the conversation. Other \vitag\/s and \reader\/s nearby will not hear anything from the requested \vitag.

\subsection{Multiple \vitag\/s to One \reader}
\label{subsec:multitagto}
When multiple \vitag\/s want to talk to one \reader\ simultaneously, every \vitag\ has to wait for it's own time slot scheduled by the \reader\ to transmit.

\subsection{Multiple \reader\/s to One \vitag}
\label{subsec:multireaderto}
One other problem is when multiple \reader\/s want to talk to one \vitag, how to arbitrate the media. To solve this problem, \reader\/s run ALOHA with carrier sensing. Specifically, if \reader\ has data to send, send the data. If, while \reader\ is transmitting data, it receives any data from another \reader, there has been a message collision, in which case all involved \reader\/s back off for an arbitrary period of time before retrying. Unlike \vitag, \reader\/s do not have a tight energy constraint, and so carrying out carrier sensing on them is possible.

\subsection{One \vitag\ to Multiple \reader\/s}
\label{onetagto}
The reverse problem is when \vitag\ wants to talk to one \reader, how it will prevent other \reader\/s in range from being interrupted. In principle, \vitag\ is supposed to respond to the polling request sent by the \reader\ that has the strongest illuminance on \vitag, so as to get the best performance. However, detecting light strength is too energy consuming for \vitag\/s. On the other hand, \reader\ does not have a tight energy budget and can assess the strength as well, of the signal backscattered by \vitag\/s, which is negatively correlated with the distance from a \vitag\ to a \reader. To provide \vitag\/s in the network with the best connection, \reader\/s estimate the accessibility of every \vitag\ in range using the feedback signal in each \vitag's time slot. Specifically, the network of \reader\/s works out a mapping between best service-providing \reader\/s and every \vitag\ in range\footnote{One could exploit the link-state routing protocol to achieve  consensus on such a mapping across \reader\/s}, and keeps this information in each \reader's "\vitag\ table". Now, as every \reader\ knows which \vitag\ to serve to get the best performance, it will send polling requests only to \vitag\/s that are in the instantaneous "\vitag\ table".

\subsection{Putting Things Together}
The discussion so far brings together the physical layer and the MAC layer of the \vitag\ system. The physical layer protocol deals with point-to-point communications on the downlink (from one \reader\ to one \vitag) and the uplink (from one \vitag\ to one \reader) as well as \vitag\ duty-cycling, \vitag\ waking-up, and error-correction. The MAC layer protocol addresses the multi-\reader\ to multi-\vitag\ problem in a way different from existing RFID or WLAN because of the different constraints. With these protocols, the networked system of \vitag\/s can provide services like Internet connection to batter-free tags in the home-area sensor network scenario, and identification service in traditional RFID scenarios, with better security guarantees. We will showcase the prototype we build for the RFID scenario, and evaluate its performances and security preservation strength. 

==> ov-bg.tex <==
\section{Requirements and Preliminaries}
\label{sec:background}

% \begin{tcolorbox}
% \para{Goal} low-power bi-directional VLC.
% \para{Overview} backscattering lights using retro-reflector, modulate with LCD. 
% \para{Retro-reflector} principles, effects, properties 
% \para{LCD modulation} 
% \para{Principles} Use analog components as many as possible (to avoid ADCs) and avoid complicated digital signal processing on the mobile end. Also, design amplifiers that work at an almost-cut-off state to save energy cost. \todo{what does this sentence mean?}
% \end{tcolorbox}


Our goal is to design a bi-directional VLC system that runs on battery-free devices like smartphones and sensor nodes. The system features an LED and a mobile device. One closed-loop communication paradigm of the system is as follows. The LED sends a packet carried on the white light it emits modulated to $1MHz$ (downlink). The \vitag\ senses the transmission and wakes up. Upon successfully receiving and demodulating the packet, the \vitag\ sends a packet back to the LED (uplink). The LED is slightly modified so as to integrate the receiver in as shown in Fig.~\ref{fig:system}.

In sending the packet, instead of generating the signal using power-consuming LEDs or other communication channels such as infrared or ultraviolet carriers, we adopt the modulating retro-reflector framework, with the combination of an LCD and a retro-reflector. Driving the LCD costs only $400-\mu W$ energy. In addition, a \vitag\ passively sends signals, thus the power consumption of which can be maintained at a low level. 

%with the help from other energy saving components. Finally,  The receiver detects any signals sent by the \vitag, and decodes the bits against noises and interferences.

In the rest of the paper, we describe the design of \retro\ that consists of a modified off-the-shelf white LED and a \vitag\ in more details.

%\p{We need a system architecture figure here}

% Our goal is to design primitives that enhance visible light communication capabilities on battery-free devices while preserving user privacy and security of both the transmitters and the receivers, with the omnipresence of readily available LEDs that serve as the lightening devices. The key challenge in achieving these is two-fold. First, devices running at visible light bands are power-intensive because of the broad bandwidth these bands can provide. Second, the noise caused by ambient signals on the visible light spectrum and the interference triggered by the the data transmitted by the system itself stays in the same band as what the receiver expects to receive at. To address these challenges, we use the following guiding principles: we use as many analog components and recycle as much energy as possible on the tag to enable the tag to transmit to the reader with a decent data rate. Also, we diminish the scattering area as much as possible by making use of directional backscattering materials of small Field of View (FoV). Such approaches, as we show in the rest of the paper, can provide an order of magnitude reduction in the power consumption of these communication primitives and in the scattering area of the signals on the backscattering channel.

% In the rest of this paper, we describe \vitag, our battery-free tag and show how it can enable backscatter communications with no battery and with a higher energy efficiency with respect to communication range than tags with LEDs on. We then describe \reader, our system that can be easily integrated onto commercial LED lights for transmitting data at no discernible flickers with dimming support and receiving with \hl{hhh dB} signal-to-interference-plus-noise-ratio (SINR). Finally, we show that our designs can be used to enable concurrent transmissions in a network of battery-free devices without the need for synchronization.



%\paragraph{Visible Light Communication} 
%Visible lights are electromagnetic waves that span frequencies roughly from 400 to 800 THz. For illumination, white LEDs are commonly used. The instantaneous On/Off feature turns LEDs into effective transmitters for visible light communication (VLC). Specifically, information bits can be embedded on the light by modulating the on/off state of the LED with on-off keying (OOK) or variable pulse-position modulation (VPPM) \cite{standard}. To receive such signals, while in some cases a cell phone camera or a digital camera will be sufficient \hl{need citations, ipsn14 and mobicom14}, photodiodes are generally used, because phone cameras can only achieve around 0.25MHz sampling rate~\cite{camera1} (in other words, low data rate), whereas photodiodes have generally higher bandwidth up to 0.5GHz~\cite{pdsheet}. Moreover, compared with a phone camera, the SNR of the photodiode is orders of magnitude higher at the same distance \hl{ipsn14}. 

%A typical way to generate white lights is to use a phosphor material to convert monochromatic lights from blue or ultraviolet to broad-band white lights, where the color of the monochromatic light depends on the band gap energy of the materials forming the p-n junction in the LED. 

%Visible lights bring safety advantages over communication waves of other common frequencies, because human eyes are much more sensitive to the strength of visible lights than the invisible TV, Wi-FI and RFID transmissions. With the LED dimming support~\cite{dimming}, a person can turn down the light if she feels of a too high brightness. In addition, radios waves at some certain frequencies are likely to hard human organs, especially to pregnant women and kids~\cite{rfidharm}, while the visible light are not.

%There are two primary ways of producing white LEDs. One is to use individual LEDs that emit three primary colors --- red, green, and blue --- and then mix all the colors to form white light~\cite{ledprin1}. The other is to use a phosphor material to convert monochromatic light from a blue or UV LED to broad-spectrum white light, much in the same way a fluorescent light bulb works~\cite{ledprin2}. In general, the wavelength of the light emitted, and thus its color, depends on the band gap energy of the materials forming the p-n junction. In materials used for LEDs, the electrons and holes recombine by a radiative transition, which produces optical emission, because there are direct band gap with energies corresponding to near-infrared, visible, or near-ultraviolet light. 





\paragraph{Retro-reflector} 
Retro-reflector is a device that operates by returning light back to the light source along the same light direction with a minimum of scattering~\cite{rr}. Retro-reflectors are widely used on road signs, bicycles, and clothing for road safety. From a microscopic view, a retro-reflector is composed of cells, each of which is a corner cube as shown in Fig.~\ref{fig:retrolcd} (e). When a light beam hits one of the cells, the light is turned around via two adjacent reflections. 



\paragraph{Modulating Retro-reflector}
Modulating retro-reflector (MRR)~\cite{mrr} consists of a retro-reflector and a modulator for optical communications. An MRR operates as a passive sources which transmits bits by varying the intensity of the reflected light beam. MRR is widely used in free space communication where the other side is a laser. Existing MRR systems~\cite{expensive,expensive2} is usually of a large size, and modulation is commonly achieved with a high-end electroabsorption modulator altering the absorption spectrum by applying an electric field. Consequently, such setting is ill-suited for our scenarios which require a low-cost solution.
\p{Need double check. It is really hard to understand the existing MRR solutions. Cannot find much material.}

LCD is \todo{polarized glass + liquid, liquid can polarize incoming light, } LCDs use the light properties of liquid crystals that are controlled by the voltage added on them. When the LCD is on, the incoming light is able to pass the LCD and hit the retro-reflector; When the LCD is off, the incoming light is rejected by the LCD. Therefore, LCDs can be used as modulators for MRRs. 
%However, one disadvantage of LCDs are their low refresh rate, e.g., 60 or 75 Hz, which is too low for data communication. Fortunately, we find \textit{LCD shutters} with much higher refresh rate (up to 1KHz \hl{cite}). Fig.~\ref{fig:retrolcd} shows the basic principle of a retro-reflector with an LCD coverage.
\begin{figure}[th]
   \centering
   \includegraphics[width=0.8\columnwidth]{link.pdf}
   \caption{Downlink and uplink.}
   \label{fig:link}
   \vskip -3mm
\end{figure}

\figref{fig:link} illustrates the modulated uplink lights using LCD. We notice that the commercially off-the-shelf LCDs are of low refreshing rate. Therefore, the symbol length is relatively much longer than the carrier waveform.


\begin{figure*}[!t]
\vskip -0.1in
\centering
{\footnotesize
\begin{tabular}{ccccc}
\epsfig{file=../illustrations/mrr1.eps, height=0.2\columnwidth} &
\epsfig{file=../illustrations/mrr2.eps, height=0.2\columnwidth} & 
\epsfig{file=../illustrations/mrr3.eps, height=0.2\columnwidth} & 
\epsfig{file=../illustrations/mrr4.eps, height=0.2\columnwidth} &
\epsfig{file=../illustrations/retroreflector.eps, height=0.2\columnwidth} \\
{(a) TX $45\degree$, RX $45\degree$} & 
{(b) TX $45\degree$, RX $135\degree$} & 
{(c) TX $45\degree$, RX $90\degree$} & 
{(d) TX $90\degree$, RX $90\degree$} &
{(e) Ideal Retro-reflector} \\
\end{tabular}
}
\vskip -0.1in
\caption{\footnotesize{\bf Illustration of the Retro-reflector.} (a) When the LED (TX) is at $45\degree$ arrival of incidence, and the camera (RX) is at $45\degree$, the retro-reflector area (on the right) is bright, the mirror area (in the middle) is dark, and the paper area (on the left) is dark. (b) When the LED is at $45\degree$, and the camera is at $135\degree$, the mirror area is bright, while the retro-reflector and the paper areas are dark. (c) When the LED is at $45\degree$, and the camera is at $90\degree$, the retro-reflector and the mirror areas are dark, while the paper area is slightly bright due to diffused reflections. (d) When the LED is at $90\degree$, and the camera is at $90\degree$, both the retro-reflector and mirror areas are bright. (e) depicts an ideal retro-reflector and how it responds to incoming lights. Our actual retro-reflector has a scattering angle as small as $5\degree$}
\label{fig:retrolcd}
\vspace{-1em}
\end{figure*}






==> principle.tex <==
\section{Our Design Principle}

Our goal is to design primitives that enhance visible light communication capabilities on battery-free devices while preserving user privacy and security of both the transmitters and the receivers, with the omnipresence of readily available LEDs that serve as the lightening devices. The key challenge in achieving these is two-fold. First, devices running at visible light bands are power-intensive because of the broad bandwidth these bands can provide. Second, the noise caused by ambient signals on the visible light spectrum and the interference triggered by the the data transmitted by the system itself stays in the same band as what the receiver expects to receive at. To address these challenges, we use the following guiding principles: we use as many analog components and recycle as much energy as possible on the tag to enable the tag to transmit to the reader with a decent data rate. Also, we diminish the scattering area as much as possible by making use of directional backscattering materials of small Field of View (FoV). Such approaches, as we show in the rest of the paper, can provide an order of magnitude reduction in the power consumption of these communication primitives and in the scattering area of the signals on the backscattering channel.

In the rest of this paper, we describe \vitag, our battery-free tag and show how it can enable backscatter communications with no battery and with a higher energy efficiency with respect to communication range than tags with LEDs on. We then describe \reader, our system that can be easily integrated onto commercial LED lights for transmitting data at no discernible flickers with dimming support and receiving with \hl{hhh dB} signal-to-interference-plus-noise-ratio (SINR). Finally, we show that our designs can be used to enable concurrent transmissions in a network of battery-free devices without the need for synchronization.

==> principle_2.tex <==
\section{Design Overview}


Our goal is to design a bi-directional VLC system that runs on battery-free devices like smartphones and sensor nodes. The system features an LED and a mobile device. One closed-loop communication paradigm of the system is as follows. The LED sends a packet carried on the white light it emits modulated to $1MHz$ (downlink). The \vitag\ senses the transmission and wakes up. Upon successfully receiving and demodulating the packet, the \vitag\ sends a packet back to the LED (uplink). The LED is slightly modified so as to integrate the receiver in as shown in Fig. \ref{system}.

In sending the packet, instead of generating the signal using power-consuming LEDs or other communication channels such as infrared or ultraviolet carriers, we adopt the modulating retro-reflector framework, with the combination of an LCD and a retro-reflector. Driving the LCD costs only \hl{xx $\mu W$} energy. In addition, a \vitag\ passively sends signals, thus the power consumption of which can be maintained at a low level. 

%with the help from other energy saving components. Finally,  The receiver detects any signals sent by the \vitag, and decodes the bits against noises and interferences.

In the rest of the paper, we describe the design of \retro\ that consists of a modified off-the-shelf white LED and a \vitag\ in more details.

\p{We need a system architecture figure here}

\begin{figure}[th]
   \centering
   \includegraphics[width=0.8\columnwidth]{link.pdf}
   \caption{Downlink and uplink.}
   \label{fig:link}
   \vskip -3mm
\end{figure}

% Our goal is to design primitives that enhance visible light communication capabilities on battery-free devices while preserving user privacy and security of both the transmitters and the receivers, with the omnipresence of readily available LEDs that serve as the lightening devices. The key challenge in achieving these is two-fold. First, devices running at visible light bands are power-intensive because of the broad bandwidth these bands can provide. Second, the noise caused by ambient signals on the visible light spectrum and the interference triggered by the the data transmitted by the system itself stays in the same band as what the receiver expects to receive at. To address these challenges, we use the following guiding principles: we use as many analog components and recycle as much energy as possible on the tag to enable the tag to transmit to the reader with a decent data rate. Also, we diminish the scattering area as much as possible by making use of directional backscattering materials of small Field of View (FoV). Such approaches, as we show in the rest of the paper, can provide an order of magnitude reduction in the power consumption of these communication primitives and in the scattering area of the signals on the backscattering channel.

% In the rest of this paper, we describe \vitag, our battery-free tag and show how it can enable backscatter communications with no battery and with a higher energy efficiency with respect to communication range than tags with LEDs on. We then describe \reader, our system that can be easily integrated onto commercial LED lights for transmitting data at no discernible flickers with dimming support and receiving with \hl{hhh dB} signal-to-interference-plus-noise-ratio (SINR). Finally, we show that our designs can be used to enable concurrent transmissions in a network of battery-free devices without the need for synchronization.
